Beyond Visual Perception: Insights from Smartphone Interaction of Visually Impaired Users with Large Multimodal Models

Large multimodal models (LMMs) have enabled new AI-powered applications that help people with visual impairments (PVI) receive natural language descriptions of their surroundings through audible text. We investigated how this emerging paradigm of visual assistance transforms how PVI perform and manage their daily tasks. Moving beyond usability assessments, we examined both the capabilities and limitations of LMM-based tools in personal and social contexts, while exploring design implications for their future development. Through interviews with 14 visually impaired users of Be My AI (an LMM-based application) and analysis of its image descriptions from both study participants and social media platforms, we identified two key limitations. First, these systems' context awareness suffers from hallucinations and misinterpretations of social contexts, styles, and human identities. Second, their intent-oriented capabilities often fail to grasp and act on users' intentions. Based on these findings, we propose design strategies for improving both human-AI and AI-AI interactions, contributing to the development of more effective, interactive, and personalized assistive technologies.

==> draft.tex <==
Beyond-Visual Perception: Insights from Real-Time Interaction Between Visually Impaired Users, Large Multimodal Models, and Human Assistants

Beyond-Visual Perception: Insights from Real-Time Interaction Between Visually Impaired Users and Large Multimodal Models 


Beyond Visual Perception: Insights from Smartphone Interaction of Visually Impaired Users with Large Multimodal Models

==> sections/1._intro.tex <==
\section{Introduction}

% People with visual impairments (PVI) rely on both AI and human assistance to understand their visual surroundings. 
People with visual impairments (PVI) face challenges in perceiving their surroundings due to the absence of visual cues. \rev{Traditional} AI-powered \rev{systems like} Seeing AI~\cite{SeeingAI2020} \rev{and} human-assisted \rev{services like} remote sighted assistance~\cite{BeMyEyes2020} \rev{have helped PVI interpret their environment and complete} daily tasks. \rev{Recent advances} in computer vision (CV) and natural language processing (NLP) \rev{have enabled AI systems to identify} objects and text \rev{in scenes while responding to photo-based queries from PVI~\cite{ahmetovic2020recog, mukhiddinov2022automatic, hong2022blind, morrison2023understanding, gonzalez2024investigating}.
%
The emergence of} large multimodal models (LMMs)~\cite{yu2023mm}, \rev{particularly} GPT-4~\cite{achiam2023gpt}, \rev{has transformed} visual question-answering (VQA) \rev{capabilities.} Researchers have begun \rev{exploring how these powerful LMMs might benefit} PVI~\cite{zhao2024vialm, yang2024viassist}. \rev{At the forefront of this development is} \textit{\bma{}} (\sbma{})~\cite{bma_usecase}, the first \rev{publicly-available} LMM-based system \rev{designed specifically to help PVI with} visual interpretation and question answering\rev{. Built on} OpenAI's GPT-4 models~\cite{achiam2023gpt}, \sbma{} offers \rev{capabilities that surpass those of} similar applications.

Prior work~\cite{adnin2024look} has investigated \rev{how PVI use and access generative AI tools,} focusing on information access, acquisition, and content creation through platforms like \bma. Our work \rev{broadens this investigation beyond} content-oriented interactions to \rev{examine} real-life scenarios \rev{involving} visual descriptions, task performance, social interactions, and navigation. By \rev{analyzing} the capabilities and limitations of LMM-based VQA systems, particularly \bma{}, we identify gaps between \rev{current} technological capabilities and \rev{PVI's} practical needs and expectations. 
This study offers timely insights into rapidly evolving LMMs \rev{while seeking broader understanding that will remain valuable as foundational knowledge even as specific technologies advance.} 

\rev{
More specifically, we explore} the following \textit{research questions}:
\begin{itemize}
    \item \textit{What are the capabilities and limitations of LMM-based assistance in the daily lives of people with visual impairments?}
    % 
    \item \textit{How do people with visual impairments mitigate these limitations?}
\end{itemize}


To answer these questions, we conducted an exploratory study \rev{using two complementary data sources. First, we interviewed} 14 visually impaired users \rev{about their experiences with \sbma. This was our primary data source. Second, we analyzed image descriptions generated by this tool that were shared by both our interview participants and users on} social media platforms (X, Facebook, Reddit, and blogposts). This \rev{secondary data source allowed us to understand PVI's lived experiences with this AI tool while capturing concrete examples of their interactions in various real-life scenarios.} 


\rev{Our study revealed} that \sbma's context-aware capabilities \rev{help participants better understand their} spatial \rev{surroundings, support} social \rev{interactions, interpret} stylistic \rev{elements, and convey} human identities. \rev{Yet} several limitations \rev{undermine} these benefits\rev{: the AI sometimes hallucinates} non-existent details, \rev{makes} subjective interpretations \rev{about} human-animal interactions and fashion \rev{choices, and misidentifies} people's age or gender. \rev{When encountering these limitations, participants draw on their spatial memory and auditory cues, apply personal judgment, or turn to human assistants.} Moreover, \rev{\sbma{} struggles to grasp users' intentions, provide} actionable support\rev{, or offer} real-time feedback. Participants compensate for this by actively guiding it through prompting, seeking human \rev{assistance}, or depending on their orientation and mobility skills.


Informed by these findings, we discuss strategies to improve handoff between PVI, the AI tool, and remote sighted assistants. We propose streamlined interactions to reduce redundancy and envision new paradigms to achieve more accurate identity recognition, improve subjective interpretations, and mitigate AI hallucinations. 
% 
We also discuss the benefits of multi-agent systems, including both human-human and human-AI collaborations, and explore future possibilities of AI-AI cooperation to aid PVI in tasks requiring specialized knowledge. 


\rev{
Our research examines how state-of-the-art AI, particularly} LMM-based systems like \sbma, \rev{creates new opportunities for PVI through advanced human-like language and vision capabilities. Rather than contrasting this tool with other VQA systems, we characterized this as a new genre of AI-driven prosthetic and identified how its early-stage usage could better align with established assistive approaches such as remote sighted assistance~\cite{lee2020emerging,kamikubo2020support,granquist2021evaluation}. 
Through detailed analysis of an AI tool's capabilities and limitations, based on rich narratives from PVI about their first-hand experiences, we provide insights into how LMM-based systems are reshaping accessibility tools. These insights help us understand how to enhance both the context awareness and intent-oriented capabilities of LMMs, laying the groundwork for future advances in intelligent, interactive, and personalized assistive technology that better serve PVI's needs.
}






==> sections/2._lit_review.tex <==
\section{Background and Related Work}


% intro to DCog: collaborative, human-powered prosthetic are DCog (RSA)
% adaptive artifact that is human-like, intelligent, is also DCog (bma)

In this section, we review the literature on AI-powered and human-assisted visual interpretation and question answering systems, as well as information needed in visual interpretations for PVI.


\subsection{AI-Powered Visual Interpretation and Question Answering Systems}


The advancements in deep learning models for computer vision and natural language processing have significantly enhanced the capabilities of AI-powered visual assistive systems\rev{~\cite{ahmetovic2020recog, mukhiddinov2022automatic}}. These systems leverage photos taken by PVI to identify objects or text within the scene, as well as respond to queries about the contents of the images\rev{~\cite{hong2022blind, morrison2023understanding}. Such applications are now widely adopted, exemplified by Microsoft's Seeing AI~\cite{SeeingAI2020}, providing support to PVI in various scenarios~\cite{gonzalez2024investigating}.}

% \sout{The advancements in deep learning models for CV and NLP technologies have significantly enhanced the capabilities of AI-powered visual assistive systems. These systems leverage photos taken by PVI to identify objects or text within the scene, as well as respond to queries about the contents of the images. For instance, Ahmetovic et al.~\cite{ahmetovic2020recog} developed a mobile app utilizing deep network models to guide PVI in capturing images and recognizing objects. Mukhiddinov et al.~\cite{mukhiddinov2022automatic} devised a fire detection and notification app for PVI using convolutional neural networks. Hong et al.~\cite{hong2022blind} created an iOS app enabling PVI to gather training images for personalized object recognition. Morrison et al.~\cite{morrison2023understanding} designed an application to teach AI to identify individualized items, aiding PVI in locating personal belongings. Gonzalez et al.~\cite{gonzalez2024investigating} introduced a scene description app utilizing Microsoft's Azure AI Vision image description API. Additionally, PVI commonly employ commercial AI-powered applications like Microsoft's Seeing AI~\cite{SeeingAI2020} to recognize objects through device cameras.}

Recent advancements in LMMs, such as GPT-4~\cite{achiam2023gpt}, have demonstrated exceptional performance in multimodal tasks~\cite{yu2023mm}, \rev{prompting exploration into their potential for assisting PVI. State-of-the-art LMMs have been leveraged to create assistive systems capable of evaluating image quality, suggesting retakes, answering queries about captured images~\cite{zhao2024vialm, yang2024viassist}, and even integrate multiple functions to assist PVI in tasks such as navigation~\cite{zhang2025enhancing} and text input~\cite{10.1145/3613904.3642939}. In the commercial domain, Be My Eyes~\cite{BeMyEyes2020} introduced the \bma{} feature powered by GPT-4~\cite{achiam2023gpt}.}

% \sout{More recently, Large Multimodal Model (LMM)~\cite{yu2023mm}, represented by GPT-4~\cite{achiam2023gpt}, have showcased remarkable proficiency in multimodal tasks. In response, researchers have begun exploring the potential of LMM in assisting PVI. Zhao et al.~\cite{zhao2024vialm} investigated the feasibility of leveraging state-of-the-art LMM to aid PVI and established a corresponding benchmark. Yang et al.~\cite{yang2024viassist} utilized LMM to develop an assistive system for answering PVI's questions about captured images, including assessing picture quality and suggesting retakes. In the realm of commercial applications, Be My Eyes~\cite{BeMyEyes2020} and OpenAI collaborated to introduce the \bma{} feature~\cite{bma_usecase}, powered by GPT-4~\cite{achiam2023gpt}, aimed at replacing human volunteers.}

% \rev{While prior research has examined the use of AI-powered visual assistive systems like Seeing AI for tasks such as reading~\cite{granquist2021evaluation} and daily routine support~\cite{kupferstein2020understanding}, these studies predate the integration of advanced LMM technologies and thus may not fully reflect the capabilities or user experience of cutting-edge systems. Although some accounts, such as Bendel’s documentation of experiences with GPT-4-based \bma{}~\cite{bendel2024can}, offer insights, they remain anecdotal and lack generalizability. This study aims to bridge this gap by conducting an in-depth investigation into the daily usage of \bma{} among 14 PVI users, offering a comprehensive understanding of its real-world applications and impact.}


Prior work has examined the use of AI-powered visual assistive systems by PVI in their daily lives\rev{~\cite{granquist2021evaluation,kupferstein2020understanding,gonzalez2024investigating}}. However, these studies did not incorporate the latest LMM technologies, thus may not fully represent the user experience of cutting-edge AI-powered systems. Bendel~\cite{bendel2024can} documented his experience with GPT\mbox{-}4\mbox{-}based \bma, yet his account remains subjective. Therefore, in-depth investigation into PVI's daily utilization of state-of-the-art AI-powered systems is imperative. 
This paper addresses this gap by exploring how 14 visually impaired users incorporate \bma, a state-of-the-art LMM-based VQA system, into their daily routines. 


% Prior works have examined the use of AI-powered visual assistive systems by PVI in their in their daily lives. For instance, Granquist et al.~\cite{granquist2021evaluation} examined the use of Seeing AI for reading tasks among PVI participants, while Kupferstein et al.~\cite{kupferstein2020understanding} conducted a diary study to investigate PVI users' incorporation of Seeing AI into their daily routines. Recently, Gonzalez et al.~\cite{gonzalez2024investigating} undertook a diary study to explore the use cases of AI-powered scene description applications. 
% However, these studies did not incorporate the latest LMM technologies, thus may not fully represent the user experience of cutting-edge AI-powered systems. Bendel~\cite{bendel2024can} documented his experience with GPT-4-based \bma{}, yet his account remains subjective. Therefore, extensive and comprehensive research into PVI's daily utilization of state-of-the-art AI-powered systems is imperative. This paper addresses this gap by investigating the daily usage of \bma{} among fourteen PVI users.


% adnin2024look
% \textcolor{red}{
% Based on prior work~\cite{adnin2024look}, this study goes beyond usability and accessibility issues to identify previously unexplored limitations of LMMs. We explore higher-level insights that inform potential future directions of LMMs even if the specific implementations evolve, and map these insights into broader Human-AI and AI-AI interactions. 
% }

% https://maitraye.github.io/files/papers/BLV_GenAI_ASSETS24.pdf





\subsection{Human-Assisted Visual Interpretation and Question Answering Systems}

Human-assisted VQA systems offer prosthetic support for PVI by facilitating connections to sighted people through remote assistance. These systems utilize image-based and video-based modalities to \rev{meet varied} needs and situations.


Image-based human-assisted VQA systems allow PVI to submit photos along with their queries and receive responses after some time. An example of this is Vizwiz, where PVI can upload images accompanied by audio-recorded questions and receive text-based answers through crowdsourced assistance~\cite{bigham2010vizwiz_nearly}. This method has been successfully applied in tasks such as reading text, identifying colors, locating objects, obtaining fashion advice, \rev{and supporting social interactions}~\cite{bigham2010vizwiz_nearly, bigham2010vizwiz, burton2012crowdsourcing,gurari2018vizwiz}. 
% Additionally, Vizwiz Social extends this functionality by linking PVI with their social networks, enabling support from friends and family members~\cite{gurari2018vizwiz}. 
However, the single-photo, single-query limitation of image-based VQA systems~\cite{bigham2010vizwiz_nearly} makes it less suitable for addressing complex or contextually deep inquiries~\cite{lasecki2013answering}.



Conversely, video-based human-assisted VQA systems facilitate real-time, interactive support, allowing PVI to receive immediate assistance tailored to their specific environmental context. This approach enables the visual interpretation of real-time scenes and supports a dynamic, back-and-forth VQA process, which is essential for addressing more specific and complex contextual inquiries effectively.
The evolution of this technology has progressed from wearable digital cameras ~\cite{hunaiti2006remote,garaj2003system,baranski2015field} and webcams~\cite{bujacz2008remote,scheggi2014remote,chaudary2017tele} to the utilization of mobile video applications~\cite{holmes2015iphone, BeMyEyes2020, Aira2020,xie2022dis,xie2024bubblecam} and real-time screen sharing technologies~\cite{lasecki2011real,lasecki2013answering,xie2023two}. 
% 
Services like Be My Eyes~\cite{BeMyEyes2020}, which connects PVI with untrained volunteers, and Aira~\cite{Aira2020}, which connects PVI with trained professional assistants, exemplify the application of video-based VQA in scenarios that require immediate feedback. These services prove effective in navigation~\cite{kamikubo2020support,xie2022dis,c4vtochi,iui,yu2024human}, 
shopping~\cite{c4vtochi,xie2023two,iui}, 
and social interaction~\cite{lee2020emerging,Caroll2020Human,lee2018conversations}. 
\rev{
In this study, we revealed specific situations where participants used human-assisted VQA systems to address limitations in \bma's assistance.
}





\subsection{Information Needed in Visual Interpretations for Visually Impaired Users}

% Either AI-powered or human-assisted visual interpretation faces the same challenge: determining what specific information is necessary for visual interpretation to meet the needs of PVI. Existing research primarily focuses on identifying what information PVI seek in descriptions of online images. For instance, the Web Content Accessibility Guidelines~\cite{caldwell2008web} offer advice on creating alternative text (alt text) for images. However, these guidelines tend to follow a one-size-fits-all approach, which can be difficult to apply effectively across different contexts. Similarly, AI-based image description tools (e.g., Seeing AI~\cite{SeeingAI2020}) also adhere to this one-size-fits-all design model.

% Previous studies~\cite{gurari2018vizwiz, gurari2020captioning} have adopted sighted volunteers to decide how images should be described for PVI. Recently, more research~\cite{stangl2020person,stangl2021going,bennett2021s} has shifted toward user-centered approaches, gathering input directly from PVI to understand their preferences for image descriptions. For example, Stangl et al.~\cite{stangl2020person} explored PVI users' preferences for descriptions across different online platforms (e.g., news sites, social media, eCommerce). Their findings indicated that the source of an image significantly impacts PVI’s information needs, with common requirements across platforms (e.g., identifying a person’s gender or naming objects), as well as source-specific details (e.g., a person’s hair color on dating websites). In a follow-up study~\cite{stangl2021going}, they discovered that PVI's image description preferences are influenced not only by the image source but also by their information goals. Additionally, while subjective interpretation may be desired in certain cases, such content is not typically included in descriptions. From an ethical perspective, Bennett et al.~\cite{bennett2021s} examined screen reader users' preferences for describing personal and others' appearances, specifically addressing when and how aspects such as race, gender, and disability should be conveyed.

% Recent research also explores the varied needs for describing information from videos. For instance, Jiang et al.~\cite{jiang2024s} investigated PVI preferences for video descriptions across different types of online content (e.g., how-to videos, educational videos, music videos). Based on their proposed design framework, they offered several recommendations for improving video accessibility. For example, descriptions for entertainment videos, like music videos, should focus more on subjects (people and animals), while how-to videos should prioritize actions and tools over the subjects. Natalie et al.~\cite{natalie2024audio} conducted interviews with PVI to better understand their customization needs for video descriptions in various aspects such as length, emphasis, speed, and voice. 

% All of these studies focus on asynchronous visual interpretation systems. When it comes to synchronous systems, such as real-time video interpretation, Lee et al.~\cite{lee2020emerging} identified specific needs for scene descriptions in remote sighted assistance (RSA). The required information in RSA descriptions includes both objective details (e.g., text, spatial information, scenery) and subjective aspects (e.g., opinions on clothing). In this study, we will examine how Be My AI processes visual information and provide design insights based on the information needed by PVI.

\rev{Both} AI-powered \rev{and} human-assisted visual interpretation face the challenge \rev{of identifying what specific information is necessary to meet PVI needs}. Existing research primarily focuses on \rev{what information PVI seek in online image descriptions}. The Web Content Accessibility Guidelines~\cite{caldwell2008web} \rev{advise on creating alternative text (alt text), but their one-size-fits-all approach limits context-specific applicability}. Similarly, AI-based \rev{tools like Seeing AI~\cite{SeeingAI2020} adhere to this uniform design model.}

\rev{Earlier studies~\cite{gurari2018vizwiz, gurari2020captioning} relied on} sighted volunteers \rev{to decide image descriptions for PVI, while recent research~\cite{stangl2020person,stangl2021going,bennett2021s,chen2024role} emphasizes} user-centered approaches. For example, Stangl et al.\cite{stangl2020person} \rev{found PVI preferences for descriptions vary by platform} (e.g., news, social media, eCommerce)\rev{, with both common needs (e.g., identifying gender, naming objects) and platform-specific details (e.g.,} hair color on dating websites). \rev{Follow-up work~\cite{stangl2021going} showed preferences also depend on users' goals, with subjective details rarely included.} Bennett et al.~\cite{bennett2021s} examined screen reader users' \rev{views on describing} race, gender, and disability \rev{in appearance descriptions.}
\rev{For video content,} Jiang et al.~\cite{jiang2024s} \rev{examined PVI preferences across genres (e.g., how-to, music videos), recommending that entertainment descriptions focus on subjects, while how-to videos prioritize actions and tools.} Natalie et al.~\cite{natalie2024audio} \rev{studied PVI needs for customization in video descriptions, such as length, speed, and voice. For synchronous systems like real-time video interpretation,} Lee et al.~\cite{lee2020emerging} identified \rev{PVI needs} in remote sighted assistance\rev{, including} both objective details (e.g., text, spatial information\rev{) and subjective input} (e.g., opinions on clothing).
In this study, we will examine how the LMM-based system processes visual information and provide design insights based on the information needed by PVI.



\rev{
% image Interpretations: 
% [1] table 2 in https://dl.acm.org/doi/pdf/10.1145/3313831.3376404?casa_token=cZV0Jj4xOEQAAAAA:DUGrnBq-QrkQdqRKALU7MBuhin-liR-tyGsr0jEUvcznLAMBTFTTPbocpCy2Em-Vqz0rYs5sTLlo
% [2] https://dl.acm.org/doi/pdf/10.1145/3441852.3471233?casa_token=4gFpHDQlYvUAAAAA:hWjcbkbuhYmJ-3x6EaNoewOQbIXG93mzA7w1agDMzwKhimO_ycUgKxl-k5_2ntWpFLZ_71W3PgOf
% [3] https://dl.acm.org/doi/pdf/10.1145/3411764.3445498?casa_token=TB9lu5AmUfsAAAAA:Hx9BiXQde88FZn_oDlHEsPKTnXDae4z5FYINoFrKG43L7Qg1M3NYnXTizwQe8M5ade9Gf2Ipw_cm

% video Interpretations: 
% [1] sooyeon's paper (used in discussion 5.2)
% https://dl.acm.org/doi/pdf/10.1145/3313831.3376591?casa_token=ATq0EXcGE2oAAAAA:pgbAj9B_z6skIcxG3IaBpFYLBQBCLpq85ZnuXoP6jb2LMFNAgXVCn0W-VFU__84OYIkWF0vSZHg1

% incremental in belowing contexts
% 1. scene description: description (what is it)
% 2. navigation: description (what is it) + directional info (where is it, how to get to the destination)
% 3. task performance: description + directional info + domain knowledge (what to do, how to do it)
% 4. social engagement:  description + directional info to navigate in social space + discreet info (don't want others to know they are using rsa)


% [2] table 4 in https://dl.acm.org/doi/pdf/10.1145/3313831.3376823

}












==> sections/3._method.tex <==
\section{Method: Data Collection and Analysis}


Our exploratory study used qualitative methods to examine how PVI use \bma, an emerging LMM technology, in their daily lives.
This section details our data collection and analysis processes.





\subsection{Data Collection}





\rev{
We gathered data from two sources: interviews as the primary data source and \sbma-generated image descriptions as the secondary data source. 
Interview data captured accounts of PVI's lived experiences with \bma, enabling participants to articulate personal interactions, challenges, and perceptions of the technology. 
The image descriptions enriched and supplemented interview data by providing concrete examples of how PVI used this tool across various contexts, from daily chores to professional tasks and travel. 


We collected the two data sources sequentially. 
First, we interviewed $14$ visually impaired users, focusing on \sbma's emerging practices in their daily lives. 
At the end of each interview, we invited participants to share their image descriptions. 
However, most participants didn't have examples to share or didn't want to share due to the demanding process or personal content sensitivity (e.g., images capturing their faces). Respecting and prioritizing participant privacy, we ensured voluntary sharing of image descriptions. Consequently, 4 participants shared their descriptions voluntarily.
% 
Meanwhile, we accessed and analyzed publicly available experiences shared by PVI on reliable online platforms. 



The combination of text-based interview data and text/visual image descriptions provided richer insights into PVI's experiences with emerging LMM technologies than either source alone would have offered. We detail our data collection process in the following section. 
}






\subsubsection{Primary Data Source: Interview Data}
We recruited 14 visually impaired participants (10 blind, 4 low-vision; 4 males, 10 females) through our prior contacts and snowball sampling.  
All participants actively used \bma{} and were primarily aged 35-40. Their occupations included three students and nine employed individuals, with two participants unemployed. 
Table~\ref{user_demographic_info} presents their demographics. 
Each participant received a \$30 gift card per session for their time and effort. 




%%%%%%%%%%%
\begin{table*}[]
\small
\caption{Participants' demographics.}
\label{user_demographic_info}
\begin{tabular}{p{0.3cm}p{0.8cm}p{0.8cm}p{4.8cm}p{2.8cm}p{3cm}p{2.1cm}}
\toprule
\textbf{ID} & \textbf{Gender} & \textbf{Age Group} & \textbf{Condition of Vision Impairment} & \textbf{Age of Onset} & \textbf{Occupation Type} & \textbf{Be My AI Usage Frequency} \\ \toprule
P1 & F & 45-50 & Totally blind, retinopathy of prematurity & Since birth & IT consultant &  3 or 4 times a day \\ \hline
P2 & F & 35-40 & Low vision, cone-rod dystrophy & Since birth & Program director in a nonprofit &  a few times a week \\ \hline
P3 & F & 30-35 & Totally blind, Leber's congenital amaurosis & Since birth & Elementary school teacher & 5 times a week \\ \hline
P4 & M & 25-30 & Totally blind, Pale optic nerves & More than 12 yrs ago & Criminal law employee & 2 to 3 times a week \\ \hline
P5 & F & 40-45 & Totally blind, retinopathy of prematurity & Since birth & Manager of digital accessibility & 2 times a day \\ \hline
P6 & F & 25-30 & Totally blind, microcephaly and detached retina & Since birth & Student & once a week \\ \hline
P7 & F & 35-40 & Low vision, retinopathy of prematurity & Since birth & Part-time employee &  2 times a week \\ \hline
P8 & M & 40-45 & Totally blind, detached retina & Since birth & Insurance & a few times a day \\ \hline
P9 & F & 30-35 & Totally blind, retinopathy of prematurity & Since birth & In-between jobs & a few times a week \\ \hline
P10 & F & 30-35 & Low vision, retinitis pigmentosa & Since birth & Student &  3 or 4 times a day \\ \hline
P11 & M & 35-40 & Totally blind, retinopathy of prematurity & Since birth & Stay-at-home parent &  3 or 4 times a day \\ \hline
P12 & M & 20-25 & Low vision, Leber's hereditary optic neuropathy & Since 14 yrs old & Student &  2 times a week \\ \hline
P13 & F & 40-45 & Totally blind, retinitis pigmentosa & Low vision since infancy, totally blind since 2021 & Human service employee &  5 times a week \\ \hline
P14 & F & 35-40 & Totally blind, retinopathy of prematurity & Since a few months old & Assistive technology specialist &  5 times a week 
\\ \bottomrule
\end{tabular}
\Description[Blind participants' demographic information about gender, age, condition of vision impairment, occupation type, and Be My AI usage frequency]{Ten blind participants are female, and four blind participants are male. Their age group ranges from 25 to 50, and their occupations include student, IT consultant, stay-at-home parent, teacher, employees in nonprofit and insurance, and assistive technology specialist. Their frequency of Be My AI usage varies from 2 times a week to 4 times a day.}
\end{table*}




\paragraph{Procedure} We conducted individual semi-structured interviews via Zoom lasting 50-76 minutes, with one or two researchers present per session. All interviews were recorded with participant consent. 

The interviews followed four main phases. 
% 
\textit{First}, we invited participants to share their personal use cases for \bma. 
To facilitate recall, we referenced Be My Eyes' common use case list~\cite{bma_usecase}, prompting participants to discuss similar experiences. 
% 
Follow-up questions were posed to further investigate their experiences with each identified use case. 
% 
\textit{Second}, participants evaluated the quality of the tool's visual interpretations, focusing on accuracy, detail level, error, and appropriateness of identity descriptions. 
% 
\textit{Third}, we explored how participants used \sbma{} among their various assistive tools, including human-assisted and AI-powered VQA systems, to understand its distinct advantages and limitations. 
% 
\textit{Finally}, we collected demographic information and inquired about participants' willingness to share copies of its visual interpretations for research analysis.








\subsubsection{Secondary Data Source: Image Descriptions Generated by \bma}
Image descriptions collected from interview participants and social media platforms served as a secondary data source to complement our interview findings. These descriptions included either text-only copies, or original images sent to \sbma{} with their corresponding descriptions. Some descriptions also included follow-up questions and responses between users and the system.


\paragraph{From Participants}


Participants were given the flexibility to select their preferred documentation method, either copying text or taking screenshots. 
% 
In total, we gathered 22 image descriptions from 4 participants, as most participants either lacked examples or were reluctant to share due to privacy concerns or the effort required in documentation.
Of these descriptions, 4 were original images alongside their descriptions, while the majority consisted of text copies -- a format participants found more manageable. 
Additionally, 6 of the 22 descriptions contained follow-up questions where participants sought clarification or additional details from the system. 





\paragraph{From Social Media Platforms}

We collected image descriptions from 4 social media platforms: X\footnote{\url{http://x.com/}}, Facebook\footnote{\url{https://www.facebook.com/}}, Reddit\footnote{\url{https://www.reddit.com/}}, and blogposts. The platforms were chosen to cover both image-sharing sites (X, Facebook) and discussion forums (Reddit, blogposts).



We used the search terms ``BeMyAI'' and ``\#bemyai'' to find relevant posts on X, Facebook, and blogposts. For Reddit, we searched for ``AI'' and ``BeMyAI'' within the r/Blind community. 



We gathered posts that met the following criteria: (i) written in English, (ii) published between September 25, 2023, the official release date of \bma, and March 31, 2024, and (iii) contained image descriptions generated by the tool. 
% 
To avoid redundancy, if identical content appeared across multiple platforms, only the earliest published post was recorded. 
If one post included multiple descriptions, each description was documented as a separate entry. 
If there were multiple posts published around the same time frame about the same topic (e.g., an X or Reddit thread), they were treated as a single entry. 



We verified the authenticity of posts by confirming that they were from either the official Be My Eyes account or from users who identified themselves as visually impaired in their profiles. These established platforms serve as reliable sources where PVI regularly share their experiences. 


In total, we collected 28 \sbma-generated image descriptions from 4 social media platforms. Of these, 23 included original images sent to \sbma{} \rev{and 5 were text-only interactions.} Fifteen descriptions contained follow-up questions that participants sent to the system for additional details or clarification. 
By platform, we collected 
(i) X: 17 image descriptions (16 with original images, 6 with follow-up questions), 
(ii) Facebook: 3 image descriptions (all with original images), 
(iii) Reddit: 3 image descriptions (1 with follow-up questions), and 
(iv) blogposts: 5 image descriptions (4 with original images, 8 with follow-up questions). 
The complete dataset is available at \href{https://bit.ly/4hqo5ve}{\textit{\textcolor{black}{https://bit.ly/4hqo5ve}}}.

\rev{This dataset, although limited in size, captures crucial insights into early user experiences with \bma. By collecting descriptions shortly after its release, we documented initial user interactions and system performance during its early phase. 
}





\subsection{Data Analysis}


We used a bottom-up approach \rev{to analyze the interview data}. The first author conducted inductive thematic analysis~\cite{braun2006using} by developing initial codes through open coding, then iteratively collating and grouping these codes into themes and categories. All authors reviewed and finalized these themes during weekly meetings (see Table~\ref{codebook} in Appendix). 



\rev{
We used a top-down approach to analyze the image descriptions. 
The first author examined each image description alongside its contextual elements: the user's follow-up questions, \sbma's responses, and the circumstances of image capture. Using the codebook derived from our interview analysis, we then analyzed these descriptions deductively. 



The following example illustrates our data analysis process from inductive to deductive approach.
During interviews, participants mentioned instances where \sbma{} initially provided general scene descriptions rather than their desired specific content, requiring participants to guide it through follow-up questions. We labeled this interaction as ``Goal Understanding Dialogue.'' 
When analyzing image descriptions, we identified similar patterns (Figure~\ref{eggshells}) and classified them under this pre-established ``Goal Understanding Dialogue'' category. 



Through this process, we first identified the system's capabilities and limitations through interview data, then complement these interview findings with specific examples from the image descriptions and subsequent conversations between users and the system.

}




==> sections/4._findings.tex <==
\section{Findings}
\label{findings}

In this section, we first explore \sbma's context-aware capabilities across diverse settings, assessing its effectiveness and constraints in interpreting physical environments, social and stylistic cues, and people's identity. 
% 
Next, we examine its intent-oriented capabilities by evaluating both the strengths and limitations of the system's ability to understand and act on users' intentions. 
% 
For each aspect, our findings unfold in two parts. In \textit{Capabilities of \bma}, we examine how PVI use the system and reveal its capabilities. In \textit{Example}, we illustrate specific scenarios that present both the challenges users faced and their adaptive strategies. 



\subsection{Context Awareness}

This section examines how \bma{} enhances user experiences across diverse environments and interactions. We analyze its roles in enhancing spatial awareness in physical settings, interpreting social and stylistic context, and conveying human identities. 
% 
Our analysis considers both the system's strengths in providing context-rich descriptions and its limitations due to technical constraints and subjective interpretations. 





\subsubsection{Physical Environments}
\label{physical_environments}


Participants used \sbma{} to enhance their perception of indoor and outdoor environments through detailed scene descriptions. 
They explored various settings, from theaters (P2) and room layouts (P3, P7, P9, P13) to holiday decorations (P5) and street views (P11, P12). While the system provides structured visual information that expands spatial awareness, its effectiveness occasionally diminishes due to AI hallucinations or requires participants' guidance for accurate scanning. 




\paragraph{Capabilities of \bma} Seven participants (P2, P3, P7, P9, P11, P13, P14) reported that the AI tool's comprehensive scene descriptions enhanced their spatial awareness. 
These descriptions often uncover spatial details previously unnoticed by users, as noted by P11, \textit{``It gives me unexpected information about things that I didn't even know were there.''} 
% 


% AI hallucinations 
However, this enhanced awareness is compromised by AI hallucinations, instances where AI incorrectly identifies nonexistent objects. 
Such errors can disrupt the user's context understanding, leading to confusion or misinterpretation of the environment. To verify \sbma's descriptions, participants either seek human assistance or rely on their pre-existing mental models of the environment. 



Participants successfully guide \sbma{} using auditory cues, particularly when locating dropped objects. They combine their hearing and spatial memory to adjust camera angles, which enables the tool to scan more accurately. 
% 
This integration of participants' auditory inputs guides and refines the system performance, leading to more accurate and useful descriptions.




\paragraph{Example 1: AI Hallucinations of Adding Non-existent Details}


Be My AI provides detailed descriptions of objects, characterizing their colors, sizes (e.g., ``small,'' ``medium,'' ``large,'' and ``tall''), shapes (e.g., ``round,'' ``square,'' ``fluffy,'' ``wispy,'' ``dense,'' and ``open lattice structure''), and spatial orientations (e.g., ``on the left,'' ``to the right,'' ``in the foreground,'' ``in the middle,'' and ``in the background''). 
% 
However, four participants (P3, P5, P11, P14) encountered AI hallucinations where the tool fabricated details in their environments. 



Participants developed two strategies to verify the accuracy: consulting human assistants and drawing on their spatial memory.
P3's experience illustrates the value of human verification. When \bma{} reported a \textit{``phantom''} object behind her, she first investigated personally, finding nothing. A human assistant then confirmed the absence of any object. 

\begin{quote}
    \textit{``Apparently, Be My AI said there was an object behind me, and there really wasn't. So, then, when I went and asked somebody, `You know what is behind me?' and they said there wasn't anything behind you in the picture.''} (P3)
\end{quote}


P5's experience demonstrates how spatial memory helps identify inaccuracies. When the system incorrectly described objects next to her dogs in her home, her familiarity with the space enabled her to recognize these errors independently. This ability to leverage environmental knowledge allows participants to detect and disregard AI hallucinations effectively. 




%%%%%%%%%%%%
\paragraph{Example 2: Need for User Support in Locating Dropped Objects}

Participants (P4, P12, P13) used \sbma's sequential \textit{``top to bottom, left to right''} descriptions to locate dropped items like earbuds and hair ties. 
% 
These descriptions provided precise locations, such as when P13 learned of \textit{``a picture of a carpet with a hair tie in the upper right hand corner,''} and when P12 discovered \textit{``the earphones are directly in front of you, between your feet.''}
Such sequential descriptions allow participants to pinpoint lost objects with greater accuracy. 



To optimize the tool's scanning effectiveness, participants first used their auditory perception and spatial memory to approximate an object's location before positioning the camera. 
This adjustment allowed the tool to focus on the intended search area, rather than random searching. 
% 
For instance, P4 utilized his \textit{``listening skills''} to detect the location of a fallen object before directing the camera to that specific spot. Similarly, P12 enhanced the camera's view of dropped earbuds by stepping back from his seat to capture a better angle of the floor. 
% 
These examples illustrate how participants synergize their understanding of the environment with the system's technological capabilities to manage tasks that require spatial awareness.








\subsubsection{Social and Stylistic Contexts}
\label{social_stylistic}


Participants leveraged \sbma{} for both social interactions and style-related decisions. 
In social settings, nine participants (P2, P4, P5, P8-11, P13, P14) used it to take leisure pictures of animals like cats, dogs, birds, and horses, to better understand and monitor animal behavior and status. 
% 
In stylistic applications, it aids in identifying clothing colors (P2, P7, P9, P13), recognizing patterns (P2, P9), coordinate outfits by matching clothes with shoes and jewelry (P2, P4, P5, P6, P12), and assessing makeup (P5, P10).
% 
This section examines the system's subjective interpretations within these contexts, highlighting its utility in enriching users’ experiences and the challenges in providing accurate, context-aware descriptions.





\paragraph{Capabilities of \bma}

\sbma{} usually concludes its descriptions by injecting subjective interpretations, which enriches users' understanding of depicted scenarios. 
These interpretations encompass people's or animal's emotional states (e.g., ``a cheerful expression on his face,'' ``smiling slightly,'' ``friendly and approachable,'' ``curious expression''), 
body language (e.g., ``his arms are open as if he is engaging in a conversation or greeting the other man''),
and the ambiance (e.g., ``peaceful and natural,'' ``serene and peaceful atmosphere,'' ``cozy and cheerful holiday vibe,'' ``warm and inviting atmosphere,'' ``the atmosphere seems to be lively and festive''). 




These subjective interpretations help participants better engage in social interactions and understand animal behavior. 
% 
Participants (P5, P9-11) specifically used the system to grasp nuances in animals' facial expressions, activities, and body language (Figure~\ref{human_animal}). P10 highlighted its utility during dog walks: \textit{``Sometimes it's hard for me to know if the dog is peeing or what the dog is doing.''}

\begin{figure}[t!]
\centering
\includegraphics[width=0.4\textwidth]{images/human animal-1.png}
\caption{\bma's description of a dog, including subjective interpretations of the dog's emotions. This screenshot was provided by P9.}
\Description{Interface of Be My AI. Top of the screen is a photo of a dog. Below the photo is the description of the dog, including subjective interpretations of the dog's emotions. This screenshot was provided by P9. The full description is as follows. The picture features a happy, cream-colored Labrador Retriever sitting in front of a vibrant backdrop of Christmas presents. The dog is wearing a festive red scarf and has a joyful expression with its tongue out. Surrounding the dog are numerous gift boxes wrapped in colorful paper with patterns of snowflakes, Christmas trees, reindeer, and traditional holiday plaid. Some presents have large bows on them. Behind the dog, to the left, is a large teddy bear with a red bow, and to the right, a black bear plush toy dressed in a plaid outfit. The setting gives off a cozy and cheerful holiday vibe.}
\label{human_animal}
\end{figure}
%%%%%%%%%%%%%% fashion
Furthermore, the subjectivity extends to fashion suggestions, with \bma{} recommending stylistically coordinated outfits based on colors and patterns, as well as assessing makeup. 
For instance, P5 employed it to check the color, placement, and overall balance of her makeup, P2 and P9 consulted it to coordinate tops and bottoms, and P12 used it to select a tie that complemented his shirt. 


However, participants noted that BMA's visual interpretations sometimes included excessive subjective elements. 
This subjective input, unverified by human, could potentially undermine the system's ability to provide accurate context awareness.  
As a result, participants preferred their own subjective interpretations or feedback from sighted assistants in contexts involving human-animal interactions and fashion choices. 




%%%%%%%%%%%%%%%%
\paragraph{Example 1: Subjective Interpretations in Human-Animal Interactions}


Participants (P2, P5) identified limitations in how \sbma{} infers animal emotions in its image descriptions, raising concerns about the accuracy of these subjective interpretations. 
For instance, P5 highlighted instances where the tool describes a dog \textit{``appears to be relaxed''} or \textit{``appears to be happy.''} 
Likewise, P2 noted its tendency to include subjective commentary, as in \textit{``That's a white cat curled up on a fuzzy blanket. She looks peaceful and happy and rested.''} 



These interpretations go beyond observable visual elements to make emotional inferences that may not reflect reality. 
% 
As a result, participants expressed a preference for objective, fact-based descriptions. 
P2 articulated a desire for less editorializing, saying, \textit{``Maybe I don't want it to editorialize, you know, maybe I just literally only want the facts of it.''}



Participants (P2, P5) stressed the importance of maintaining human agency in interpreting animal behaviors, preferring their own judgment rather than the system's subjective interpretations. 
P5 particularly valued the ability to modify \sbma's descriptions of her dog's expressions, maintaining control over her interpretation of pet behaviors. 


\begin{quote}
    \textit{``Some blind people think, `How does it know that the dogs are happy? Why does it assume?' Some people don't like that it's making assumptions about the picture. I like having access to that information, but I like to be able to change it if I want.''} (P5)
\end{quote}


In summary, \sbma's subjective inferences can enrich descriptions, yet they risk introducing inaccuracies that undermine the system's reliability. Users therefore value the ability to override these interpretations, preserving their agency in understanding the context. 




\paragraph{Example 2: Subjective Interpretations in Fashion Help}


\sbma's subjective interpretations extend beyond human-animal interactions to fashion help. 
Participants (P6, P7, P10) utilized it to describe colors and patterns but expressed concerns about its subjective fashion suggestions. 
% 
They preferred to make their own style choices or seek human assistance for outfit matching, highlighting the human subjectivity in fashion decisions.



P6 questioned the AI's capacity to authentically replicate human judgment, saying, \textit{``It's interesting how AI is being taught to simulate kind of the human factor of things.''}
% 
She cited experiences where AI-generated responses appeared \textit{``strange''} and \textit{``complete nonsense,''} contrasting these with the nuanced understanding that humans provide.  



\begin{quote}
    \textit{``No, no, no, no, I would never use it to do anything that required human subjectivity... I just don't trust AI with a task that is supposed to be subjective like that, particularly visual like that. Have you ever seen AI weirdness?... I think that just goes to show why I'm not gonna trust AI with my fashion yet.''} (P6)
\end{quote}


P10 explicitly preferred human feedback, stating, \textit{``I'm still more confident asking a sighted person to provide me with the feedback.''} 
This preference underscores how participants maintain their agency by relying on human judgment for fashion decisions rather than deferring to \sbma's suggestions. 







%%%%%%%%%%%%
\subsubsection{Identity Accuracy and Sensitivity}
\label{identity}


Nine participants (P2, P3, P5-7, P9-11, P13) evaluated the system's ability to describe people's identities in images of their families, friends, and social media posts. 
Our analysis examines how the tool handles identity attributes like age and gender, focusing on both its capabilities and limitations in providing sensitive and accurate descriptions. 




\paragraph{Capabilities of \bma}

\sbma{} describes people's identity in terms of gender (e.g., ``woman,'' ``man''), age (e.g., ``old,'' ``late twenties or early thirties''), appearance (e.g., ``long, dark brown hair,'' ``wavy brown hair,'' ``His hair falls past his ears, with a slightly messy but stylish look'') and ethnicity (e.g., ``East Asian''). 
% 
Participants appreciated such detailed descriptions for providing deeper insight into people's visual characteristics. P2 explained: \textit{``I enjoyed hearing, I knew my friend was East Asian when I saw her picture. It was kind of cool to see that because... as a blind person, you don't know that all the time. So, I'd like access to it.''}


However, eight participants (P2, P3, P5-7, P9, P10, P13) encountered challenges with the system's accuracy and sensitivity in describing identity attributes, particularly gender and age. 
% 
These errors reveal the tool's limited ability to interpret contextual cues that extend beyond visual appearance, such as cultural, situational, and personal contexts. 



\paragraph{Example: Inaccurate Identification of People's Gender and Age}


Three participants (P3, P10, P13) reported inaccuracies in \sbma's gender identification. 
P13 described how it misidentified gender by mistaking a hidden ponytail for short hair: \textit{``just looked like short-cropped hair.''} 
% 
Similarly, P10 revealed that the system struggled with gender identification for individuals whose physical attributes do not conform to typical gender norms, noting, \textit{``the person had a short hair, and was a female''}. 
In response, it defaulted to neutral language, \textit{``\bma{} didn't tell me it was a woman or a man, just said a person.''}
% 
These examples illustrate the system's reliance on stereotypical indicators and reveal its challenges in interpreting non-visible details.



Additionally, two participants (P5, P9) identified problems with age description. P9 reported that \bma{} overestimated her daughter's age by one year. 
% 
Likewise, P5 observed sensitivity concerns when the system labeled someone as \textit{``an old woman''} based solely on grey hair. 
% 
To address these age-related inaccuracies, P5 suggested that the tool should adopt more objective, factual descriptions rather than subjective or potentially stigmatizing labels, such as \textit{``a woman with grey hair, instead of an older woman.''}
% 
These examples indicate the system's difficulties with precise age estimation and the potential inaccuracy when AI makes assumptions based on appearance alone.



In summary, these examples illustrate the tool's limited context awareness and its challenge in accurately interpreting people's identities, such as gender and age, due to the reliance on stereotypical visual cues. These misjudgements are rooted in the system's inability to integrate and interpret broader, non-visible contextual elements like cultural norms and personal styling choices. 








%%%%%%%%%%%%%
%%%%%%%%%%%%%
\subsection{Intent-Oriented Capabilities}

In this section, we explore \sbma's limitations \rev{in} comprehending users' goals, providing actionable support to fulfill these objectives, and offering real-time feedback. 
% 
Through analysis of specific examples, we elucidate the extent of the system's intent-oriented capabilities and highlight areas where it falls short in adapting to user needs. 



\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{images/cooking - eggshell.png}
\caption{On the left is the original image sent to \bma. On the right is \bma's description of eggs in a frying pan, followed by a question checking for the presence of eggshells. This example was originally drawn from X.}
\Description{On the left is the image of a frying pan on the stove-top. Inside the pan there are 4 eggs, one of whose yolk is broken. On the right is a photo of an user using Be My AI on a smart phone.}
\label{eggshells}
\end{figure}


\subsubsection{Agentic Interaction}
\label{agentic_interaction}

While \bma{} can process visual information, it often struggles to infer users' specific intentions from images. Users compensate for these limitations by guiding the system through targeted prompting. 


\paragraph{Capabilities of \bma}



BMA's ``ask more'' function enables users to explore image details that were not covered in initial descriptions. Through this feature, users can probe for specific details that match their personal needs or interests.
% 
Eleven participants (P1-3, P5, P6, P8-12, P14) used the ``ask more'' function to 
match outfits (P2, P5, P12),
check makeup (P5, P10), 
suggest cooking recipes (P12), 
assist with household appliances (P5, P12), 
examine text or objects (P6, P8, P11, P12, P14),
gain more details about people's facial expressions, attire, or actions (P2, P3, P5, P8, P9, P10, P11), 
check animal status (P3, P5, P11, P14), 
and edit the descriptions for social media posts (P2, P3). 



Seven participants (P1-3, P5, P8-10) valued the flexibility of posing follow-up questions, enhancing their independence by reducing reliance on human assistance. As P3 noted, \textit{``I can ask follow-up questions, so I have a good way to sort of figure out what's in the image independently, which is something I was not able to do before this app came out.''} 


However, participants identified a common issue that the system is unable to discern users' goals in initial response, often resulting in generalized descriptions without knowing which aspects to emphasize. P12 elaborated on this challenge, stating, \textit{``\bma{} loves to make general descriptions, and it doesn't know what to focus on.''} 
To overcome this limitation, users guide the system with targeted prompts that clarify their specific intentions. 





\paragraph{Example 1: Check for the Presence of Eggshells}







In Figure~\ref{eggshells}, BMA's initial response provides a detailed descriptions of what is included in a frying pan. 
The user, likely influenced by prior experiences of inadvertently leaving unwanted items in the pan while cooking, specifically intended to check for such elements. 
% 
However, the system did not infer that the user was looking for unwanted elements like eggshells, rather than seeking a general description of the scene.
% 
To clarify her objective, the user posed a follow-up question, thus directing \sbma{} to recognize and prioritize her specific concerns and intentions. 



In this example, although the AI tool can describe the visual elements accurately and comprehensively (from the condition of the eggs to the surroundings), it failed to identify unusual visual elements that are challenging for PVI to detect but are important to their understanding of the scene. 
% 
User prompting helps refocus the system's attention on these unusual elements, thereby enhancing its ability to interpret and respond to user-specific intents more effectively. 



%%%%%%%%%%
\paragraph{Example 2: Adjust Rotary Control Appliances}
Six participants highlighted the tool's inadequacy in comprehending their goal of adjusting rotary control appliances like washers (P1) and thermostats (P2, P4, P5, P13, P14). This task requires \bma{} to interpret the current settings on these appliances as users modify dials for time, mode, or temperature.
% 
However, the system often offered broad descriptions of visual elements without honing in on the user's specific objectives. 


P13's experience exemplifies this limitation. While the system could recognize a thermostat on the wall, it failed to provide critical information such as the current temperature setting or instructions for adjusting the temperature. 



To overcome the limitation, participants guided the system to better understand their goal through prompting. 
% 
For instance, P5 asked precise questions like \textit{``What is the arrow pointed at right now on the current setting?''} Such specific queries helped redirect \sbma's focus from general scene descriptions to the exact details needed for appliance adjustment. 





\subsubsection{Consistency and Follow-Through}
\label{consistency}


In Section~\ref{agentic_interaction}, we described how users needed to explicitly guide \bma{} when it failed to understand their intentions. 
% 
This section examines the system's difficulties maintaining consistency and following through on tasks even after acknowledging users' goals. 



\paragraph{Capabilities of \bma}


\sbma{} often fails to proactively suggest next steps or support users until they achieve their objectives. 
% 
Effective consistency requires maintaining focus on the user's objective throughout the interaction. \rev{This includes} offering progressively specific and relevant assistance, and ensuring all responses contribute to the user's intended outcome.


Due to these limitations, participants turn to human assistants. \rev{Human assistants} can interpret the context of tasks and goals more dynamically, \rev{providing} conversational guidance and adapting to users' actions to facilitate goal completion. 




%%%%%%%%%%%%
\paragraph{Example 1: Inadequacy in Identifying Central Puzzle Piece}

P14 used \sbma{} to differentiate between various puzzles by describing the images on the boxes like a scene of cats or bears. 
% 
When tasked with identifying the centerpiece of a nine-piece puzzle using the box image, \sbma{} failed to provide the necessary detail for this precise task. 
% 
Initially, the system correctly read text from the puzzle box indicating which piece belonged in the center. 
However, when P14 requested more specific guidance to locate the centerpiece, \sbma{} only noted that it was square -- a characteristic shared by multiple pieces. This response was too vague for successful puzzle assembly. 



\begin{quote}
    \textit{``When \bma{} read me the text of the box on the back of the puzzle that said, you know, this particular piece should be in the center of the puzzle. As a follow-up question I asked, `Could I have more information about the piece in the center?' And it said, `This piece is a square piece,' but I mean, there were many different square pieces, so I could not tell from that.''} (P14)
\end{quote}
% 
This example illustrates the system's limited ability to translate visual understanding into actionable guidance. While it could process the image and comprehend users' general goals, it could not provide the detailed information needed for successful goal achievement. 
As a result, P14 turned to a family member for assistance. 


\begin{figure}[t!]
\centering
\includegraphics[width=0.6\columnwidth]{images/description-of-a-conference-room.png}
\caption{\bma's description of a conference room, with the original image cropped. This example was drawn from X.}
\Description{Screenshot of the Be My AI interface. In the top is the description of a conference room. In the bottom left is the Take Picture button. In the bottom right is the Ask More button. The full description is as follows. The picture shows an indoor conference room with a group of people seated at round tables. The attendees appear to be focused on something at the front of the room, which is not visible in the photo. The room has a wooden floor and a ceiling with white beams, from which stage lights are hanging. The tables are covered with grey tablecloths, and there are some papers and bottles on them. There's a screen visible in the background showing some kind of presentation or logo, but it's not clear what it is. The lighting in the room is bright, and the overall atmosphere seems professional.}
\label{incomplete_info}
\end{figure}
% \footnotetext[2]{\url{https://x.com/Chr1sLew1s/status/1732730506557477052}}

\paragraph{Example 2: Lack of Instruction for Camera Adjustment}
\label{adjust_camera}

A common challenge for participants (P3, P5, P6, P8, P10-12, P14) was aligning the camera properly to capture clear views of their intended areas. 
\bma{} can identify image quality issues, notifying users when pictures were \textit{``cut off''} (P5), \textit{``blurry''} (P6), or incomplete (Figure~\ref{incomplete_info}).  
% 
However, it is unable to provide further actionable guidance on adjusting the camera to improve image clarity. 
% 
This limitation manifested in scenarios where \sbma{} recognized both the user's goal of capturing specific areas and the image deficiencies but could not suggest practical solutions. 
As P6 described, \textit{``It was very frustrating because it said the picture is blurry. Can you please put the label in the frame? But I didn't know how to put the label on the frame.''} 








%%%%%%%%%%%%%
Eight participants (P1-3, P7, P8, P12-14) \rev{resolved this challenge by turning to human assistants, who can offer} adaptive support to achieve their goals, \rev{especially in} tasks that require continuous feedback. P13 shared an example where a human assistant not only understood her goal but also guided her in adjusting the camera and instantly reminded her to turn on the light to achieve her objective.

\begin{quote}
    \textit{``You know, having that ability to communicate and say, `Hey, this is what I'm looking for.' Or one time, I was looking for something and I had the lights off, and they're like, `You need to turn the lights on.' And I go, `Okay,' as opposed to, you know, if I tried using AI for that, it would just say `dark room.'''} (P13)
\end{quote}


This example highlights human assistants' ability to adapt their communication based on the situation and the user's implied needs, providing solutions that directly support achieving the user's goals.
% 
\rev{However}, \bma{} struggles to provide practical assistance despite understanding basic requests. 







\subsubsection{Real-Time Feedback}
\label{realtime_feedback}

We investigate how participants used \sbma{} to support navigation tasks, focusing on location awareness and orientation. 
Our analysis reveals the system's constraints in delivering real-time feedback and comprehensive navigational information from static images, and its inability to facilitate immediate interactions with surroundings.  



\paragraph{Capabilities of \bma}

Participants (P2, P5, P10) employed \sbma{} to aid in localization and orientation while navigating to their destinations. 
% 
For instance, P2 utilized it to identify gate numbers at the airport, P5 employed it to read signage directing toward the airport's transportation area, and P10 used it to recognize her surroundings when disoriented in her neighborhood.  
% 
Despite these benefits, participants encountered challenges when using \sbma{} for navigation. The primary limitations stemmed from the limited camera view and practical mobility issues. 




\paragraph{Example 1: Limited Navigational Information in Static Images}


Six participants (P2, P5, P6, P10, P11, P13) reported that \sbma's reliance on static images rather than real-time videos makes it difficult to capture comprehensive navigational information, such as obstacles and signage, in a single shot. 
% 
As P6 described, users \textit{``have to stand there and keep taking pictures and taking pictures,''} verify the captured content, assess its utility for navigation, and adjust the angle for additional shots. This iterative process can be time-consuming, \textit{``It'll be too much of a task that's supposed to take maybe 10 minutes would probably take like 30.''}



P10 elaborated on the challenge and risk of simultaneously taking pictures and navigating, particularly when attempting to identify and navigate around obstacles. The uncertainty of capturing all potential hazards was a significant concern. 



\begin{quote}
    \textit{``It's still hard to know how to capture, you know, all the obstacles. I think that's the issue. Like, how to know that I captured the right obstacle on my path? I mean, it depends [on] what I'm able to capture with the camera. You know, that's the tricky part for somebody without vision to capture the obstacle.''} (P10)
\end{quote}


Given these limitations, participants preferred human assistance through video-based interactions over \bma{} for real-time navigation. 
Video interactions not only benefit from human adaptability in adjusting guidance (Section~\ref{adjust_camera}) but also offer crucial real-time feedback unavailable in static images. 
Participants (P2, P6, P13) suggested that real-time video interpretation capabilities would significantly enhance the system by eliminating the need for repeated picture-taking. 



\begin{quote}
    \textit{``If you could hold the camera and it could do it in real time, versus having to stop, take a [picture], then assess it... If that were the case, then you could move on to doing things like uploading videos and getting it to describe actual videos and things like that, versus just still images. That would be great. You know, then you could describe more.''} (P2)
\end{quote}
% 
Such real-time video analysis would enable continuous camera movement and immediate feedback, streamlining the navigation process without pausing and reviewing individual images. 



%%%%%%%%%%%%%%
\paragraph{Example 2: Irreplaceable Role of Orientation \& Mobility Skills in Navigation}


Besides the value of real-time visual interpretations from external resources like human assistants, participants (P5, P10, P13, P14) emphasized the indispensable role of real-time feedback through their Orientation and Mobility (O\&M) skills for safe navigation.
% 
P5 and P13 pointed out that even human assistance, though adaptive in guiding PVI away from navigational hazards, cannot substitute for essential O\&M skills required for tasks like street crossing.
Consequently, participants are more cautious about relying on emerging AI tools for navigation.
% 
P14 reinforced this perspective, saying, \textit{``it's not a replacement for our mobility skills or just any skills in general. It can aid and augment the skills but it's not a replacement for them. It shouldn't be.''} 



%%%%%%%
Participants (P5, P13) further delineated vital information provided by O\&M skills or discerned through O\&M tools like white canes or guide dogs, which current AI or human assistance cannot replace. 
First, immediate surroundings. \bma{} can identify obstacles \textit{``that are a little far away''} (P5) but may miss immediate surrounding hazards. 
Second, distance and proximity measurements of obstacles. Although \sbma{} can indicate the presence of obstacles, it lacks the capability to measure their distance.
Third, directional details. Essential navigational information, such as the direction of stairs (ascending or descending) or the presence of railings, are not always detectable through the system. 
% 
With the O\&M skills and tools, users can instantly adapt their movements based on direct interaction with their environment. This level of responsiveness is currently unattainable with AI tools or human assistance. 


\begin{quote}
    \textit{``[\bma] says, you know, `stairs in front,' and it's like, `Okay, that's great, but where are they? How far are they? Are they going up? Are they going down? Is there a railing?' which would be information that the dog or the cane could tell you. So, I would say use it as a tool along with, but definitely not by itself.''} (P13)
\end{quote}


In summary, neither AI systems nor human assistants can replace the essential, real-time feedback and adaptive capabilities offered by O\&M skills and tools. These elements are vital for ensuring safe navigation by allowing users to directly interact with their environment.


==> sections/5._discussion.tex <==
\section{Discussion}
\label{sec:discussion}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\textwidth]{images/discussion_eggshell_user+app_combined.pdf}
\caption{The top shows the status quo of handoff between the user and \bma. The bottom illustrates our proposed simplified interaction.}
\Description{The top figure illustrates the current state of interactions between the user and Be My AI, where the user submits a photo and Be My AI returns a response in the first time of interaction. Subsequently, the user poses a follow-up question to Be My AI and Be My AI returns a more detailed description in the second time of interaction. The bottom figure is our proposed simplified interaction, where Be My AI learns from previous interactions and returns a detailed description during the first interaction, without user asking follow-up question.}
\label{fig.discussion_eggshell_user+app}
\end{figure*}




In this section, we examine the current state of handoff between users, \bma, and remote sighted assistants, and propose new paradigms to address the challenges identified in our findings. 
Next, we explore how multi-agent systems, both human-human and human-AI interactions, assist visually impaired users, and envision the transition toward AI-AI collaborations for tasks requiring specialized knowledge. Finally, we discuss the potential advantages of real-time video processing in the next generation of AI-powered VQA systems.






\subsection{Handoff Between Users, \bma, and Remote Sighted Assistants}
\label{handoff}

In this study, we illustrated the advantages of the latest LMM-based VQA system in (i) enhancing spatial awareness through detailed scene descriptions of objects' colors, sizes, shapes, and spatial orientations
(Section~\ref{physical_environments}), (ii) enriching users' understanding in social and stylistic contexts by detailing emotional states of people or animals, their body language, ambiance
(Section~\ref{social_stylistic}), and identity recognition (Section~\ref{identity}), 
and (iii) facilitating navigation by interpreting signages (Section~\ref{realtime_feedback}). 


Informed by our findings, despite these various benefits, there are challenges that the system alone cannot overcome.  
\bma{} still requires human intervention, either from the blind user or the remote sighted assistant (RSA), to guide or validate its outputs.  
% 
Users seek confirmation from RSAs or depend on their own spatial memory to overcome AI hallucinations, where \sbma{} inaccurately adds non-existent details to scenes. Users also rely on auditory cues and spatial memory to locate dropped objects and direct the system toward the intended search areas (Section~\ref{physical_environments}).
% 
Moreover, users actively prompt the system to understand their specific objectives, such as checking for eggshells in a frying pan or adjusting appliance dials (Section~\ref{agentic_interaction}). 
% 
There are also instances where users require assistance from RSAs when the system fails to provide adequate support to fulfill users' objectives, such as identifying the centerpiece of puzzles or adjusting the camera angle (Section~\ref{consistency}).
% 
Human assistance or users' O\&M skills are necessary to receive real-time feedback for safe and smooth navigation (Section~\ref{realtime_feedback}). 



Furthermore, our findings revealed that the system might produce inaccurate or controversial interpretations. Users express skepticism towards \sbma's subjective interpretations of animals' emotions and fashion suggestions (Section~\ref{social_stylistic}), and have encountered inaccuracies in \sbma's identification of people's gender and age (Section~\ref{identity}). These instances underline potential areas where human judgment is necessary to corroborate or correct the system's descriptions.





Next, we discuss the handoff~\cite{mulligan2020concept} between users, \bma, and RSAs to mitigate the aforementioned challenges. 




% \begin{figure}[]
% \centering
% \includegraphics[width=0.95\textwidth]{images/discussion_eggshell_user+app.png}
% \caption{Status quo of handoff between the user and \bma.}
% \label{fig.discussion_eggshell_user+app}
% \end{figure}


% \begin{figure}[]
% \centering
% \includegraphics[width=0.95\textwidth]{images/discussion_eggshell_user+app-single-interaction.png}
% \caption{Status quo of handoff between the user and \bma.}
% \label{fig.discussion_eggshell_user+app}
% \end{figure}






%%%%%%%%%%%%%
\subsubsection{Status Quo of Interactions Between Users and \bma}


Through BMA's ``ask more'' function, users are able to request additional details about the images that were not covered in initial descriptions. 
% 
This functionality facilitates a shift in interaction dynamics between users and \bma, even if the system may not accurately understand or answer users' questions in the first attempt. 
In these interactions, users are not merely passive recipients of AI-generated outputs, they actively guide the AI tool with specific prompts to better align AI's responses with their objectives. 


Our findings reported one instance where the AI tool fails to grasp the user's intent to check the presence for eggshells in the beginning (Figure~\ref{fig.discussion_eggshell_user+app} top). First, the user submits an image of eggs in the pan. Respond to the image, the system describes the quantity and object (``Inside the frying pan, there are three eggs'') and states of the yolks and whites (``whites separated'', ``yolk has broken'', ``mixing with the egg white''). Next, the user clarifies her inquiry by asking, ``are there any shells in my eggs?''
This prompts the system to understand the user's goal, reevaluate the image, subsequently confirming the presence (``Yes, there is a small piece of eggshell in the frying pan'') and location of an eggshell to help her remove it (``near the bottom left of the broken egg yolk''). 


This interaction exemplifies the status quo of handoff, where the user and \bma{} engage in a back-and-forth dialogue to refine the descriptions based on the ``ask more'' function and the user's precise prompts. 
% 
\rev{While this iterative process allows the system to eventually understand the users' intent without RSAs' intervention, it places cognitive burden on users who must carefully craft and iteratively refine their prompts. The cognitive load increases as users mentally track what information they've already received, analyze gaps between their needs and the system's responses, and develop increasingly specific queries. 
}






\rev{To reduce users' cognitive load, we propose enabling the system to adopt a mechanism that combines multi-source data input with long-term and short-term memory capabilities~\cite{zhong2024memorybank}. With explicit user consent, future versions of LMM-based VQA systems could integrate data from users' mobile devices (e.g., location information, time data) alongside historical interaction data within the system (e.g., contexts and follow-up questions) to recognize user preferences and common inquiries, and infer their needs, thereby generating responses more effectively in similar contexts. Long-term memory serves as a repository for capturing generalized user preferences, behavior patterns, and aggregated insights across multiple users. This long-term memory is particularly effective for improving system intelligence by identifying common user needs and optimizing general responses~\cite{priyadarshini2023human}. Meanwhile, short-term memory can focus on task-specific optimization within a single interaction session. It retains context from the immediate conversation, such as recent user inputs and system responses, to enhance relevance and coherence in real time. Short-term memory operates dynamically, clearing retained data once the session ends or the task is completed, thereby ensuring privacy and preventing unnecessary data retention.}


% However, this interaction could be further simplified by training \bma{} to learn from previous dialogues. By recognizing user preferences and common inquiries, such as identifying unusual elements in the scenario (eggshells in cooking eggs), we envision that the system could proactively address user concerns more efficiently and thus reduce the need for multiple clarifying prompts (Figure~\ref{fig.discussion_eggshell_user+app} bottom). 
\rev{For example, when identifying unusual elements during cooking (e.g., eggshells in cooking eggs), \bma{} could utilize the user's immediate input while referencing short-term memory from the current session or recent similar interactions. Additionally, by leveraging long-term memory, the system can learn from the user's past questions and query patterns to better match their habits and preferences, i.e., user's typical needs. Furthermore, multi-source data input, such as time or location information, can assist the system in inferring the user's current context, for instance, recognizing that the user is preparing a specific meal at a particular time or place, which allows the system to provide more relevant and context-aware assistance. This approach enables \bma{} to proactively anticipate user intent and deliver targeted responses, reducing the need for multiple clarifying prompts (Figure~\ref{fig.discussion_eggshell_user+app} bottom).} 

\rev{Cognitive Load Theory (CLT) suggests that well-designed interactions can significantly reduce users' extraneous load while enhancing the effective management of germane load~\cite{sweller1988cognitive, chandler1991cognitive}. Following the principles of CLT, we recommend using the above design to enable LMM-based VQA systems to minimize unnecessary clarifying prompts, thereby reducing users' cognitive load. 

}






\begin{figure*}[h!]
\centering
\includegraphics[width=0.8\textwidth]{images/discussion_eggshell_user+app+rsa.png}
\caption{Handoff between the user, \bma, and RSA for identity interpretations.}
\Description{The user submits a photo of people to Be My AI. Be My AI recognizes the requirement for identity interpretations and direct the photo to a remote sighted assistant. The remote sighted assistant returns a description of people's identities to Be My AI. Be My AI learns from the assistant's responses.}
\label{fig.discussion_eggshell_user+app+rsa}
\end{figure*}



%%%%%%%%%%%%%

\subsubsection{AI Deferral Learning for Identity Interpretations} 
\label{sec:deferral_learning}
% 


Our findings elucidated \sbma's capabilities and limitations in interpreting identity attributes. Although the system can describe aspects like gender, age, appearance, and ethnicity, it may make errors due to its reliance on stereotypical indicators and its inability to interpret non-visible details (Section~\ref{identity}).
% 
However, Stangl et al.'s work~\cite{stangl2020person} pointed out that PVI \rev{seek identity interpretations from AI assistants} across various contents, including \rev{browsing} social networking sites where our participants reported using \bma.


% human's ability 
This reveals a tension between PVI's interests in knowing about \rev{identity} attributes and the AI's challenges in providing reliable information\rev{~\cite{hanley2021computer}}. The conflict arises because attributes such as age and gender are not purely perceptual and cannot be accurately identified by visual cues alone. \rev{However}, RSAs \rev{can draw on contextual clues, past interactions, and cultural knowledge to make more nuanced observations about these human traits.} These social strategies are not typically accessible to AI systems. 
% \rev{This suggests a need for human-AI collaboration: certain tasks are best handled by AI assistants, others by human assistants, and still others through coordinated effort between both~\cite{gonzalez2024investigating}.}


% To mitigate these issues, we consider the potential benefits of AI \rev{deferral} learning that involves handoff between the user, \bma, and RSA. The process is illustrated in Figure~\ref{fig.discussion_eggshell_user+app+rsa}.

% To facilitate effective handoff between AI and human assistants,
To mitigate these issues, \rev{we propose adopting a deferral learning architecture~\cite{mozannar2020consistent, raghu2019algorithmic}, where an AI model learns when to defer decisions to humans and when to make decisions by itself. As detailed by Han et al.~\cite{han2024uncovering} and illustrated in Figure \ref{fig.discussion_eggshell_user+app+rsa}, this architecture creates a three-stage information flow:


\begin{itemize}
    \item \textbf{Stage 1}: It begins when users submit image-based queries to \bma. At this stage, the system uses a detection mechanism to identify sensitive contents, focusing particularly on those involving human physical traits. Current large-language models have already incorporated such mechanisms~\cite{perez2022red, bai2022training}; however, they still struggle to interpret human identity with consistent accuracy~\cite{hanley2021computer}.    
    
    % 
    \item \textbf{Stage 2}: Rather than declining sensitive requests outright, \bma{} redirects these queries to RSAs. This maintains the system's helpfulness while ensuring accurate responses. 
    % 
    \item \textbf{Stage 3}: RSAs provide descriptions by leveraging contextual understanding, such as analyzing the users' current environment and cultural background.
    % Additionally, RSAs employ a variety of social strategies by integrating contextual information, historical interactions, and cultural insights to deduce user attributes and preferences, ensuring that responses are not only relevant but also culturally and contextually appropriate. 
    % RSAs provide detailed descriptions by leveraging contextual understanding and social awareness.    
    %\textcolor{red}{RSAs can employ a variety of social strategies to deduce these attributes by leveraging context, prior interactions, and cultural insights.} 
\end{itemize}




In contrast to prior work that addresses stereotypical identity interpretation through purely computational approaches~\cite{wang2019balanced,wang2020towards,ramaswamy2021fair}, our proposed AI deferral learning takes a hybrid human-AI approach that combines AI capabilities with human expertise. 
% 
While previous AI-only solutions have made progress in reducing bias, they still struggle with identity interpretation~\cite{hanley2021computer}.
The challenges arise not only from technical issues but also from the ontological and epistemological limitations of social categories (e.g., the inherent instability of identity categories), as well as from social context and salience (e.g., describing a photograph of the Kennedy assassination merely as ``ten people, car'').
%
Our system leverages RSAs who have got more experience and probably more success in identifying people's identity through their human perception abilities and real-world experience. 
RSAs can interpret subtle contextual cues, understand cultural nuances, and adapt to diverse presentation styles that may challenge AI systems. 
% For example, RSAs can understand cultural markers of identity, and perceive age and ethnicity across different cultural contexts. 
Through the AI deferral learning architecture, AI assistants can learn continuously from human assistants' responses and improve its ability to handle similar situations. The three-way interactions between users, AI assistants, and RSAs generate rich contextual data that can enhance the AI system's identity detection mechanisms.} 

% Such process could also be adapted for requests involving the interpretation of social contexts \rev{like assessing animals' emotions (Section~\ref{social_stylistic})}. It can facilitate \bma{} continuously improve through observation and learning from human expertise. 

% When equipped with memory capabilities and given user consent, the AI assistant can build a knowledge base of individuals whom users frequently encounter. Moreover, the three-way interactions between users, AI assistants, and RSAs generate rich contextual data that can enhance the AI system's identity detection mechanisms.



% compared to prior works attempted to address the issues of stereotypical identity interpretation, how does the proposed AI referral learning could perform better?
% \textcolor{red}{[add prior work on identity interpretation (e.g., CV)]}

% \textcolor{red}{referral, when handoff to human,  challenges of ai referral learning is how to get the dataset. here bma get the dataset for training from rsa.}


% \rev{
% In contrast to prior work that addresses stereotypical identity interpretation through purely computational approaches~\cite{wang2019balanced,wang2020towards,ramaswamy2021fair}, our proposed AI referral learning takes a hybrid human-AI approach that combines AI capabilities with human expertise. 
% % 
% While previous AI-only solutions have made progress in reducing bias, they still struggle with identity interpretation~\cite{hanley2021computer}.
% The challenges arise not only from technical issues but also from the ontological and epistemological limitations of social categories (e.g., the inherent instability of identity categories), as well as from social context and salience (e.g., describing a photograph of the Kennedy assassination merely as ``ten people, car'').
% %
% Our system leverages RSAs who have got more experience and probably more success in identifying people's identity through their human perception abilities and real-world experience. 
% RSAs can interpret subtle contextual cues, understand cultural nuances, and adapt to diverse presentation styles that may challenge AI systems. For example, RSAs can understand cultural markers of identity, and perceive age and ethnicity across different cultural contexts. 
% Through the AI referral learning framework, \bma{} can learn from RSAs' nuanced interpretations in these scenarios, gradually improving its ability to handle similar situations. The system logs RSAs' responses and uses them as training examples, allowing \bma{} to develop more context aware in identity recognition. 
% }
% % 
% Such referral learning processes could also be adapted for requests involving the interpretation of social contexts. It can facilitate \bma{} continuously improve through observation and learning from human expertise. 


\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\textwidth]{images/discussion_eggshell_user+app+rsa-check.png}
\caption{Handoff between the user, \bma, and RSA for fact-checking.}
\Description{The user submit a photo to Be My AI, Be My AI returns a description with possible AI hallucination. Then, the user directs the photo to a remote sighted assistant, who returns a corrected description to the user.}
\label{fig.discussion_eggshell_user+app+rsa-check}
\end{figure*}


%%%%%%%%%%%%%
\subsubsection{Fact-Checking for AI Hallucination Problem}
% ai hallucinations - informed by our findings, cannot be addressed, ask humans 



Our findings highlighted that the AI-generated detailed descriptions helped users understand their physical surroundings. However, there were instances where AI systems hallucinated, i.e. incorrectly added non-existent details to the descriptions, which led to confusion (Section~\ref{physical_environments}). 
% 
\rev{
In fact, hallucinations is a known problem for large language models upon which \bma{} is built~\cite{gonzalez2024investigating}. Current approaches to address this problem include Chain-of-thought (CoT) prompting~\cite{wei2022chain}, self-consistency~\cite{wang2022self}, and retrieval-augmented generation (RAG)~\cite{lewis2020retrieval}.
% 

In CoT prompting~\cite{wei2022chain}, users ask an AI model to show its reasoning steps, like solving a math problem step by step rather than simply giving the final answer. It is similar to the ``think aloud'' protocol in HCI. 
% 
Self-consistency~\cite{wang2022self} is an extension of CoT prompting. Instead of generating just one chain of thought, the model is asked to generate multiple different reasoning paths for the same task. Each reasoning path might arrive at a different answer. The model then takes a ``majority vote'' among these different answers to determine the final response.
% 
In RAG~\cite{lewis2020retrieval}, AI models are provided with relevant information retrieved from a vector storage as ``context'' to reduce factual errors in their responses.
}

\rev{
In light of these techniques, users adopt various strategies that mirror CoT prompting, self-consistency, and RAG. We outline some potential strategies below.
% with a visual (Figure~\ref{fig.discussion_eggshell_user+app+rsa-check}).
\begin{itemize}
    \item \textbf{Part-Whole Prompting}: This strategy parallels the Chain of Thought (CoT) prompting. A user sends an image to \bma{} and requests an initial overall description, followed by a systematic breakdown that justifies this description. For example, users might first ask for a description of the image as a ``whole'', then request to divide the image into smaller ``parts'', like a $3 \times 3$ grid, and describe each grid individually. If the descriptions of the individual parts align coherently, it increases the likelihood that the overall description is accurate. This approach would require processing more information; however, it will provide users with greater confidence in the AI's response, as it enables them to verify consistency between the whole and its constituent parts.  
    % 

    \item \textbf{Prompting from Multiple Perspectives}: This strategy resembles the self-consistency technique. A user sends an image to \bma{} and requests multiple descriptions from different perspectives. For example, users might ask for one description that focuses on the background and another that emphasizes foreground objects. Users can also request descriptions from the viewpoint of objects within the image (e.g., ``How would a person sitting on a chair see this scene?'' and ``How would a person sitting on the floor see this scene?''). While gathering descriptions from multiple perspectives may increase the likelihood of hallucination, it can also help identify common elements that appear consistently across different viewpoints, potentially indicating true features of the image.    
     % 
    \item \textbf{Prompting with Human Knowledge}: This strategy resembles the RAG approach. A user sends an image to \bma{}, provides their current understanding of the image and its context, and requests a description that complements their knowledge. For example, in Figure~\ref{eggshells}, users can specify that someone took the picture in a kitchen environment and that it should show a frying pan containing eggs. Users possess this knowledge through their familiarity with physical environments, self-exploration, spatial memory, and touch~\cite{gonzalez2024investigating}. The user-provided knowledge will help the AI model ground its response in an accurate context~\cite{liu2024coquest}.     
    % 
    \item \textbf{Pairing with Remote Human Assistants}: While the previous three strategies rely on multiple prompting and response aggregation to identify facts, this approach leverages the traditional remote sighted assistance framework.
    This strategy (shown in Figure~\ref{fig.discussion_eggshell_user+app+rsa-check}) differs from the deferral learning framework (Section~\ref{sec:deferral_learning}) in that users forward the AI responses to human assistants, rather than the AI assistant deferring to humans for the response.
    In this strategy, a user first sends an image to \bma{} to receive a description. When users suspect inaccuracies through triangulation~\cite{gonzalez2024investigating}, such as descriptions that conflict with their spatial memory or common sense (e.g., implausible objects like a palm tree in a cold region), they can request a RSA to fact-check the description. The RSA then verifies the description and sends corrected information back to the user. This verification process is likely easier and faster for a RSA than composing a description from scratch, as the RSA's work involves checking rather than creating content.
\end{itemize}
}

\rev{
In summary, AI hallucination presents both challenges and opportunities. By addressing these issues, future work will strengthen the way users, AI models, and human assistants interact with each other.
}















%%%%%%%%%%%%%
%%%%%%%%%%%%%
\subsection{Towards Multi-Agent Systems for Assisting Visually Impaired Users}


%%%%%%%%%%%%
This section examines the transition from human-human interactions to human-AI and AI-AI systems in supporting PVI. We explore how these multi-agent systems, which involve the collaborative efforts of multiple agents (AI or human), are designed to adaptively meet the diverse needs of PVI. 


Lee et al.~\cite{lee2020emerging} identified four contexts in which a professional human-assisted VQA system (Aira) offer support to PVI. The type of information required by PVI is incremental in these contexts. 
First, \textit{scene description} and \textit{object identification} acquire information about ``what is it.''
Second, \textit{navigation} requires description about PVI's surroundings and obstacles (``what is it'') and directional information (``where is it'' and ``how to get to the destination'').
Third, \textit{task performance} like putting on lipstick, cooking, and teaching a class. This context requires description (``what is it'') and domain knowledge on ``how to do it.'' 
% directional information (``where is the intended object'' and ``how to get it''), as well as
Forth, \textit{social engagement} like helping PVI in public spaces or interacting with other people. This needs description (``what is it''), directional information to navigate in social space, and discreet communication (PVI prefer not to disclose their use of VQA systems).


Our study reported how participants used \bma{} for tasks like matching outfits and assessing makeup, fitting under the category of \textit{task performance}. Some participants raised concerns about the accuracy of \sbma's interpretations and suggestions, indicating their preference for human subjectivity in this context. 
% 
Contrasting with this, Lee et al.'s work~\cite{lee2020emerging} highlighted that remote sighted assistants (RSAs), even those professionals RSAs from Aira, sometimes lack the specialized information or domain knowledge required in task performance, thereby they need to collaborate with other RSAs to find solutions. 


Furthering this investigation, Xie et al.~\cite{xie2023two} paired two RSAs to assist one visually impaired user in synchronous sessions, validating the need for RSAs to complement each other's description in task performance like aiding the user in applying makeup and matching outfits. They also explored the challenges in this human-human collaboration, revealing collaboration breakdowns between two opinionated RSAs. 
% 
To address these issues, they proposed a collaboration modality in which one ``silent'' RSA supports the other RSA by researching but not directly communicating. This approach suggested that two RSAs in this multi-agent system should not deliver information simultaneously but have a clear division of labor, designating who takes the lead, to avoid overwhelming PVI with information. 


% AI-RSA handoff (section 5.1) to AI-AI (GPT + expert AI)
Transitioning from human-human to human-AI collaboration, the handoff between the user, \bma{} and RSA (Section~\ref{handoff}) opens up new opportunities for multi-agent systems. 
% 
Our proposed modality of human-AI collaboration integrates the scalable, on-demand capabilities of AI-based visual assistance with the contextual understanding and adaptability of RSAs. 
This multi-agent system involves the AI system recognizing its own limitations and seamlessly handing off tasks to a RSA when appropriate. This collaboration aligns with prior work~\cite{xie2023two}, where AI (\bma) and human (RSA) maintain a clear division of labor, minimizing cumbersome back-and-forth and reducing potential confusion for PVI. 



Looking ahead, we envision the potential for AI-AI collaboration as part of the future multi-agent systems to assist PVI, especially for task performance. 
A domain-specific AI expert can be trained to handle more specialized tasks such as matching outfits, performing mathematical computations, or answering chemistry-related questions. \bma, as the core AI system, can provide general visual descriptions (``what is it'') and delegate more specialized tasks requiring domain knowledge to the domain-specific AI expert. 
% 
This approach is in line with the human-AI collaboration (Section~\ref{handoff}) by ensuring effective handoffs when necessary. By leveraging AI agents with more specialized capabilities, this multi-agent system can better adapt to PVI's needs. 



However, similar to concerns around human-human and human-AI interactions, these AI-AI collaborations must be carefully designed with clear protocols and handoff points for transitioning tasks between AI agents. It is important to make these transitions as seamless and transparent as possible to PVI, thereby avoiding any complexity or confusion. 




%%%%%%%%%%%
%%%%%%%%%%%
\subsection{Towards Real-Time Video Processing in LMM-based VQA Systems}


One of the most significant advantages of \bma{} and other LMM-based assistive tools is their ability to provide contextually relevant and personalized assistance to users. By leveraging machine learning and natural language understanding, these systems can understand and respond to a wide range of user queries. This level of contextual awareness represents a significant advancement over pre-LMM-based assistive technologies, which often fail to adapt to the diverse needs and preferences of individual users.


However, our findings also identified several challenges and limitations associated with the reliance on static images by current LMM-based assistive tools. 
Participants in our study reported frustration with the need to take multiple pictures to capture the desired information, a process they found time-consuming and cognitively demanding (Section~\ref{realtime_feedback}). This iterative process hinders efficiency and also poses safety risks, as participants struggled with taking images while navigating around obstacles.


% \rev{[real-time video process can also facilitate the transition from conveying ``what'' to ``how'' questions]}
To mitigate these issues, integrating real-time video processing capabilities into future LMM-based VQA systems could offer significant benefits. 
% 
Our findings suggest that the dynamic nature of video serves as a foundation for subsequent guidance (Section~\ref{realtime_feedback}), which is currently provided by human assistants through video-based remote sighted assistance.
% 
Shifting to real-time video processing would allow LMM-based VQA systems to transition from identifying objects (answering ``what is it'') to offering practical advice (addressing ``how to do it''), such as how to adjust the camera angle or how to navigate to a destination.
% 
By continuously analyzing the user's surroundings through real-time video feeds, these systems can dynamically interpret changes and provide immediate feedback, thus eliminating the need for static image captures. This capability would enhance the user experience by offering seamless navigation aid in real time. 


The feasibility of real-time video processing is supported by existing technologies demonstrated in commercial products and research prototypes. For instance, systems that utilize sophisticated algorithms for real-time object segmentation in video streams~\cite{wang2021swiftnet} have shown significant potential in other domains. Building on these techniques for video analysis could significantly extend the capabilities of future LMM-based VQA systems. 


Transitioning from static image analysis to real-time video processing can alleviate the burden of iteratively taking pictures and adjusting angles experienced by users. It can also enhance the utility and safety of LMM-based VQA systems, particularly during navigation. 
% 
This progression, driven by ongoing advancements in machine learning and computer vision, is essential for the development of more adaptive and responsive assistive technologies that align with the dynamic nature of real-world environments.




% Our findings highlight a limitation in the capabilities of \bma{} when it comes to providing actionable, goal-oriented guidance to PVI (Section~\ref{appliances}). While \bma{} is good at conveying ``what'' information with most of time accurately describing the visual content of a scene or object, such as identifying a thermostat on the wall. 
% 
% It often struggles with providing ``how'' information, guiding users on the specific actions required to interact with or operate elements in their environment, such as how to adjust the theromstat. This ``what'' and ``how'' divide poses a major challenge to the effectiveness and usability of \bma{}, as PVI rely on it not only for understanding their surroundings but also for completing tasks and achieving their goals.



% To address this limitation and design more goal-oriented AI-powered assistant prosthetics, we propose the following key design implications. 
% % 
% Future AI-powered assistive technologies should be designed with a focus on action-oriented reasoning and task-specific guidance. Although this could be achieved through further user inquiries~\cite{truhn2023large}, integrating knowledge bases~\cite{zhu2014reasoning} and event/behavior reasoning engines~\cite{chen2008using} to enable contextual inference of actions and intentions, and associating visual elements' feedback with reasoning, would greatly reduce the cognitive burden on PVI and enhance the user experience. By leveraging this knowledge, assistive technologies can provide more relevant and actionable guidance to PVI, helping them effectively navigate and interact with their environment to complete desired tasks. Our findings emphasize the importance of human-centered design principles, particularly in the design of assistive technologies, which should be reinforced through a goal-oriented technical roadmap that adapts to users' needs, preferences, and external environments~\cite{fischer2001user,amershi2014power}. By emphasizing action goal-oriented reasoning~\cite{huffman1993goal,letier2002agent}, future AI-powered prosthetics will be optimized, further benefiting PVI.






% reference about real-time image processing:
% By continuously analyzing the user's surroundings and providing relevant information without the need for explicit image capture, these systems could offer a more seamless and efficient user experience. The integration of \textcolor{red}{real-time image processing} into AI-powered VQA systems aligns with the growing availability of commercial products and research prototypes that leverage advanced object detection and text recognition technologies. For example, Microsoft's Seeing AI \cite{SeeingAI2020} and various currency recognition systems \cite{liu2008camera, parlouar2009assistive, paisios2012exchanging} demonstrate the feasibility and potential impact of real-time image processing in assistive technology. By building upon these existing approaches and incorporating state-of-the-art deep learning techniques for object detection \cite{girshick2014rich, girshick2015fast, ren2016faster, krizhevsky2017imagenet} and text recognition \cite{ma2018arbitrary, he2017deep, zhou2017east, yao2016scene, liu2017deep, lyu2018multi}, future AI-powered VQA systems could provide even more robust and reliable assistance to users.







% \subsection{Subjectivity Interpretations}
% % positive, identity
% know gender, race, humans have problem in identifying it, humans also guess but not make public mistake. not purely perceptual. discussion: neutral, conflict. tension between prior work and this one. only objective info and pvi will use social skills. intent in physical social gathering - limitations of prior work, digital interactions
% % https://dl.acm.org/doi/10.1145/3313831.3376404



% % negative, social cues
% [Discussion:] ai, human agency, undermine pvi as people, they can understand the social meanings. compare to human agents, subjectivity comes from ai no verification 








% \subsection{Design Implications for AI-Powered Assistant Prosthetics} %Albert
% % Design Implications: How AI-Powered Visual Question Answering Should Look Like
% As demonstrated by our research, \bma{} has shown significant potential in empowering PVI by providing a more intuitive, user-friendly, and context-aware assistive experience. However, to further enhance the usability and effectiveness of AI-powered VQA systems like \bma{}, several design implications should be considered.
% %lmm: large multi model 
% %
% %Suggest features that could improve \bma's usability, like real-time image processing to reduce the need for multiple pictures.
% %
% %Recommend design changes that might help \bma become more goal-oriented and contextually aware, such as advanced machine learning models trained on diverse environments.



% \subsubsection{Towards Goal-Oriented AI-Powered Assistant Prosthetics}

% %bma good at what information (``what'' is about the visual content) but not ``how'' information
% %
% %(Section~\ref{appliances}) recognize thermostat (what), but not adjust dial (how)

% Our findings highlight a limitation in the capabilities of \bma{} when it comes to providing actionable, goal-oriented guidance to PVI (Section~\ref{appliances}). While \bma{} is good at conveying ``what'' information with most of time accurately describing the visual content of a scene or object, such as identifying a thermostat on the wall. 
% % 
% It often struggles with providing ``how'' information, guiding users on the specific actions required to interact with or operate elements in their environment, such as how to adjust the theromstat. This ``what'' and ``how'' divide poses a major challenge to the effectiveness and usability of \bma{}, as PVI rely on it not only for understanding their surroundings but also for completing tasks and achieving their goals.

% To address this limitation and design more goal-oriented AI-powered assistant prosthetics, we propose the following key design implications. 
% % 
% Future AI-powered assistive technologies should be designed with a focus on action-oriented reasoning and task-specific guidance. Although this could be achieved through further user inquiries~\cite{truhn2023large}, integrating knowledge bases~\cite{zhu2014reasoning} and event/behavior reasoning engines~\cite{chen2008using} to enable contextual inference of actions and intentions, and associating visual elements' feedback with reasoning, would greatly reduce the cognitive burden on PVI and enhance the user experience. By leveraging this knowledge, assistive technologies can provide more relevant and actionable guidance to PVI, helping them effectively navigate and interact with their environment to complete desired tasks. Our findings emphasize the importance of human-centered design principles, particularly in the design of assistive technologies, which should be reinforced through a goal-oriented technical roadmap that adapts to users' needs, preferences, and external environments~\cite{fischer2001user,amershi2014power}. By emphasizing action goal-oriented reasoning~\cite{huffman1993goal,letier2002agent}, future AI-powered prosthetics will be optimized, further benefiting PVI.
 


% \subsubsection{Towards Real-Time Processing AI-Powered Assistant}
% One of the most significant advantages of \bma{} and other LMM-based assistive tools is their ability to provide contextually relevant and personalized assistance to users. By leveraging the power of machine learning and the ability for understanding of natural language, these systems can understand and respond to a wide range of user queries. This level of contextual awareness represents a significant advancement over traditional assistive technologies, which often struggle to adapt to the diverse needs and preferences of individual users.

% However, our findings also identify several challenges and limitations of current LMM-based assistive tools, particularly in terms of their reliance on user-generated images. Participants in our study reported frustration with the need to take multiple pictures to capture the desired information, which can be time-consuming and cognitively demanding (Section~\ref{navigation}). To address this issue, we envision the integration of real-time image processing capabilities into future AI-powered VQA systems. By continuously analyzing the user's surroundings and providing relevant information without the need for explicit image capture, these systems could offer a more seamless and efficient user experience. The integration of real-time image processing into AI-powered VQA systems aligns with the growing availability of commercial products and research prototypes that leverage advanced object detection and text recognition technologies. For example, Microsoft's Seeing AI \cite{SeeingAI2020} and various currency recognition systems \cite{liu2008camera, parlouar2009assistive, paisios2012exchanging} demonstrate the feasibility and potential impact of real-time image processing in assistive technology. By building upon these existing approaches and incorporating state-of-the-art deep learning techniques for object detection \cite{girshick2014rich, girshick2015fast, ren2016faster, krizhevsky2017imagenet} and text recognition \cite{ma2018arbitrary, he2017deep, zhou2017east, yao2016scene, liu2017deep, lyu2018multi}, future AI-powered VQA systems could provide even more robust and reliable assistance to PVI.



% \subsubsection{Towards Reliable AI-Powered Assistant Prosthetics}



% Our findings highlight the significant potential of AI-Powered assistive technologies like \bma{} in enhancing the perception and understanding of surroundings for PVI. However, our study also reveals a notable drawback of AI-powered assistant prosthetics, namely AI hallucinations. These errors, where the artifact inaccurately identifies objects that aren't present, can lead to confusion and mistrust among users. Participants in our study reported instances where \bma{} erroneously added non-existent details to scenes (Section~\ref{scene}). 
% It can be argued that the presence of AI hallucinations poses a major challenge to the reliability and robustness of AI-powered assistive prosthetics. If users cannot trust the information provided by these systems, their effectiveness as cognitive extensions is severely compromised. This issue is particularly critical for PVI, who rely on these technologies to navigate and make sense of their environment.

% To address the problem of AI hallucinations, our participants applied various strategies, such as consulting human assistants for verification or relying on their own knowledge to identify inaccuracies. While these strategies showcase PVI's adaptability and problem-solving skills, they also highlight the need for more reliable and robust AI-powered assistive technologies.

% One potential approach to mitigating AI hallucinations is to incorporate uncertainty estimation and communication into the design of these technologies. By quantifying and conveying the confidence level of predictions, AI-powered assistive systems can help users assess the reliability of the information provided. This approach has been explored in the context of other AI-based systems, such as medical diagnosis~\cite{leibig2017leveraging,begoli2019need} and autonomous vehicles~\cite{michelmore2018evaluating}.

% Another strategy is to develop AI-powered assistive technologies that can learn and adapt to user feedback over time. By allowing PVI or human assistants to correct errors and provide input to improve system performance, which is not only able to continuously improve system's reliability and robustness and also help aware users about possible AI hallucinations. This approach aligns with the principles of interactive machine learning, emphasizing the importance of human-in-the-loop learning for AI systems~\cite{amershi2014power,retzlaff2024human}.

% In addition to these technical solutions, involving PVI in the design and evaluation of AI-powered assistive technologies is crucial. By engaging users as co-designers and co-evaluators, researchers and designers can gain a better understanding of the challenges and requirements of PVI, leading to the development of more reliable and robust systems. This participatory design approach has been widely advocated in the assistive technology domain~\cite{frauenberger2015pursuit,lee2004trust,zhang2023redefining}.




% \subsubsection{Envisioning Multimodal AI-Powered Assistant Prosthetics} 

% %integrate multimodal input, participants can use gestures, touch, haptic feedback to interact with \bma. 

% %llm

% Our research demonstrates the superior ability and performance of \bma{} compared to previous AI-powered systems when handling various tasks. In tasks such as object recognition, processing complex information, and interpreting graphical elements, \bma{} not only completes the tasks but also provides extended explanations and further task collaboration capabilities. 
% This undoubtedly greatly expands the interaction scenarios and user experience of \bma{}. 

% However, as mentioned earlier, the current \bma{} faces challenges, including higher interaction costs due to multiple photo captures and AI hallucinations.
% % previously mentioned, we found that the current \bma{} still has some challenges and limitations in terms of interaction experience, such as the additional interaction costs caused by the need for multiple photo captures and AI hallucinations.
% % 
% Apart from integrating additional advanced technologies to expand \bma{}'s capabilities, we also suggest adopting multimodal interaction. This approach, a key design insight from our research, underscores the value of diverse interactions and feedback in AI-powered assistive tools.
% % apart from integrating other advanced technologies to expand \bma{}'s capabilities, we suggest introducing the concept of multimodal interaction, which is another key design implication derived from our research, emphasizing the importance of multimodal interaction and feedback in artificial intelligence assistive tools. 
% % 
% Although \bma{} primarily relies on voice-based input and output, integrating multimodal interaction methods, such as touch, gestures, and haptic feedback, will greatly enhance the usability and accessibility of LMM-based assistive functions. This perspective of combining multimodal interaction has been widely studied in some previous literature \cite{turk2014multimodal, reeves2004guidelines}.
% % oviat2017handbook
% For example, touch-based gestures can enable users to navigate the system interface more effectively, while haptic feedback can provide additional spatial and contextual information to supplement voice output. These multimodal interactions also allow \bma{} to adapt and personalize to better meet the diverse needs of PVI. Future research should further explore how to design and implement these multimodal interaction technologies and assess their long-term impact on PVI user experience and quality of life.

% %Our research demonstrates the superior ability and performance of \bma{} compared to previous systems and tools when handling various tasks. For instance, in tasks such as object recognition, processing complex information, and interpreting graphical elements, \bma{} not only accomplishes the tasks but also provides \textcolor{red}{multimodal input,} extended explanations, and further task collaboration capabilities. This undoubtedly greatly expands the interaction scenarios and user experience of \bma. Traditional applications and tools, such as those using conventional OCR technology and rapid reading applications like ``Seeing AI,'' are considered effective. \textcolor{red}{[cite:] However, users find it challenging to process a complete task flow using such tools, as their functions are designed for single tasks.} In other words, traditional applications and tools can only complete a specific step in a task flow and cannot connect the context of the entire task. Leveraging the LMM's ability to understand multimodal data, interact using natural language, and be context-sensitive, \bma{} can comprehend more practical needs and provide personalized assistance to users based on their requirements. Furthermore, \bma{} demonstrates its potential to replace previous assistive methods and technologies. \textcolor{red}{This is particularly evident in a series of scenarios where \bma{} substitutes RSA services, such as when participants use \bma{} for reading and control tasks. These tasks, which are considered replaceable by \bma{}, are common needs of PVI in RSA services. }

% %Another key design implication that emerged from our research is the importance of multimodal interaction and feedback in AI-powered assistive tools. While \bma{} primarily relies on voice-based input and output, \textcolor{red}{participants expressed interest in exploring other interaction modalities, such as touch, gestures, and haptic feedback.=> integrate other interaction modalities, such as touch, gestures, and haptic feedback, into \bma} The incorporation of multimodal interaction techniques, which have been extensively studied in the HCI literature \cite{turk2014multimodal, reeves2004guidelines, oviatt2017handbook}, could greatly enhance the usability and accessibility of LMM-based assistive tools. For example, touch-based gestures could enable users to navigate the system's interface more efficiently, while haptic feedback could provide additional spatial and contextual information to supplement voice output.

%\subsubsection{future ai assistant prosthetic}
%from 5.4, about design process? 
%
%integrate new tech: generative ai 
%next iteration




% \subsubsection{Opportunities in Human-AI Collaboration}
% % Evolution of Human-AI Collaboration
% % Future AI Assistant Prosthetic - From Temporal Dimension to Consider Design Implications
% Again, while our findings demonstrate the significant potential of AI-powered assistive technologies in enhancing PVI's capabilities across various contexts, participants also highlighted some limitations of these technologies. However, we argue that these limitations may be part of an adjustment period as PVI learn to interact with and adapt to AI-powered assistive technologies.


% This observation aligns with the findings of~\citet{10.1145/3563657.3595977}, who described how users, when initially using AI-powered assistive technologies, may encounter responses that do not match their expectations. Despite this, most participants were able to quickly learn and adapt to the system, reaching a point where they could collaborate with \bma{} to complete tasks and perceive it as an effective technology.

% This contradictory state may give rise to a form of Human-AI ``confrontation.'' However, this ``confrontation'' appears to diminish as the system undergoes iterative upgrades and PVI update their understanding of the system's capabilities. From a phenomenological perspective, Ihde's theory~\cite{ihde1991instrumental} suggests that the science of tools evolves alongside people's cognition, implying that the relationship between PVI and AI-powered assistive technologies is not static but rather a dynamic process of mutual adaptation and growth.


% As PVI become more familiar with the capabilities and limitations of AI-powered assistive technologies, they develop strategies to leverage these technologies effectively and compensate for the shortcomings. This process of adaptation and learning is a critical aspect of the distributed cognition framework, which emphasizes the role of artifacts and the environment in shaping cognitive processes \cite{hollan2000distributed}.


% Moreover, the iterative nature of AI-powered assistive technologies, with ongoing updates and improvements, allows for a continuous refinement of the Human-AI interaction. As these technologies become more sophisticated and attuned to the needs and preferences of PVI, the initial ``confrontation'' may give way to a more seamless and synergistic collaboration between PVI and AI-powered assistive technologies.

% This perspective highlights the importance of considering the temporal dimension of design implications in the context of AI-powered assistive technologies. Rather than viewing the limitations of these technologies as static barriers, we should recognize the potential for PVI to adapt and develop new cognitive strategies in response to these limitations, and for the technologies themselves to evolve in response to user feedback and needs.


%%%%%%%%%%
% \subsubsection{Ethical Considerations and User Involvement in the Design of AI-Powered Assistive Technologies}
% As we continue to explore the potential of AI-powered assistive technologies for PVI, it is crucial to involve the target users in the design and evaluation process \cite{10.1145/3025453.3025899}. Our research with \bma{} underscores the importance of actively engaging with PVI throughout the design process to ensure that these systems are tailored to their specific needs, preferences, and contexts of use. By involving users as co-designers and co-evaluators, we can create assistive tools that are not only technologically advanced but also truly empowering and inclusive.

% Moreover, the development of AI-powered assistive technologies should be guided by a commitment to ethical and responsible innovation~\cite{floridi2018ai4people,jobin2019global}. As LMM-based systems become increasingly sophisticated and integrated into users' daily lives, it is essential to consider issues of privacy, security, and fairness. Researchers and designers should ensure these technologies are transparent, accountable, and aligned with the values and goals of the communities they serve~\cite{10.1145/3351095.3372873}.

% In conclusion, our research with \bma{} highlights the immense potential of LMM-based assistive tools for PVI while also revealing key design implications for future AI-powered VQA systems. By integrating real-time image processing, supporting multimodal interaction and feedback, and prioritizing user-centered design principles, we can create assistive technologies that are more usable, effective, and empowering. As the field of AI-powered assistive technology continues to evolve, it is essential for HCI researchers and practitioners to collaborate with PVI's communities to ensure that these innovations are developed in an inclusive, ethical, and responsible manner.



%\subsection{\textcolor{red}{Most assistive technologies die after their introduction}}
%
%\textcolor{red}{[combine with design implications, with sub-headings]}

%Assistive technologies for PVI have undergone a rapid evolution in recent years~\cite{10.1145/3597638.3608412}, with the introduction of LLM-based applications like \bma{} marking a significant shift in the landscape. \textcolor{red}{Traditional assistive technologies, such as VQA}~\cite{bigham2010vizwiz_nearly,BeMyEyes2020}, screen readers and braille displays~\cite{muhsin2024review,alves2009assistive}, have long been the primary methods for blind individuals to access the content and navigate the world. However, assistive technology is undergoing a transition from human-driven to AI-driven~\cite{xu2023transitioning, 10.1145/3234695.3239330}, and the emergence of a series of technology-dominated assistive services has challenged the dominance of these traditional technologies, offering a more intuitive, user-friendly, and versatile experience for blind users. Our research further reveals that \bma{} has elevated AI-led assistive technology to new heights, which inevitably leads one to imagine the possibility of a future where assistive technology is fully AI-dominated.
%
%Despite the initial promise and potential of many traditional assistive technologies, a significant number of them gradually lost their appeal after the emergence of applications like \bma{}, and may eventually die out after users fully adopt \bma{}. This phenomenon can be attributed to several factors, including the lack of comprehensive functionality, high complexity of operation, social difficulties and limited usage scenarios~\cite{gori2016devices,manjari2020survey,tapu2020wearable}. These technologies failed to meet the evolving needs and expectations of blind users in one or more aspects, while \bma{} seems to offer a promising solution that integrates and expands the capabilities of various traditional assistive technologies.
%
%
%While \bma{} is not perfect at present, the introduction of \bma{} represents a significant milestone in the development of assistive technologies for blind individuals. These applications offer new possibilities and empower PVI in unprecedented ways. Building on this foundation, it is crucial to approach their development and adoption from a user-centered perspective, ensuring that they are accessible, inclusive, and responsive to the diverse needs of the blind community~\cite{10.1145/3025453.3025895,federici2012assistive}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%this paragraph can be removed.
%The rise and fall of traditional assistive technologies, coupled with the emergence of LLM-based applications \bma{}, offer valuable lessons for the future development and adoption of assistive tools for PVI. First and foremost, user-centered design and continuous adaptation must be at the heart of assistive technology development to ensure that these tools truly meet the evolving needs and expectations of blind users. Second, the success of LLM-based applications highlights the importance of leveraging advanced technologies, such as natural language processing and machine learning, to create more intuitive and versatile assistive tools. Finally, the challenges and concerns surrounding the adoption of LLM-based applications underscore the need for ongoing research, collaboration, and dialogue among researchers, developers, and blind users to ensure that these technologies are developed and deployed in an accessible, inclusive, and responsible manner.


%The introduction of \bma{} represents a significant milestone in the evolution of assistive technologies for blind people. While these applications offer new possibilities and empower blind individuals in unprecedented ways, it is crucial to approach their development and adoption with a user-centered perspective, ensuring that they are accessible, inclusive, and responsive to the diverse needs of the blind community. As the field of assistive technology continues to evolve, researchers and developers must remain committed to creating tools that truly enhance the lives of blind individuals and promote their full participation in the digital world. %The decline of traditional assistive technologies in the face of LLM-based applications serves as a reminder of the importance of continuous innovation, adaptation, and user-centered design in the quest to create a more accessible and inclusive world for all.





==> sections/6._conclusion.tex <==
\subsection{Limitations} 


There are \rev{some} limitations of this work.
First, we completed the interviews prior to March 2024 and gathered \sbma's image descriptions from its official release until March 31, 2024. Thus, our analysis did not encompass versions of \bma{} released after March 2024. Given the frequent updates and evolution of the system, there may be feature changes or enhancements introduced post-March 2024 that were not considered in our study. Future research can investigate the capabilities and limitations of newer versions of \bma{} to provide updated insights.  
% 
\rev{Second, while our focus on initial user experiences provided insights into early-stage interactions with \bma, this early-phase data collection resulted in a limited dataset. Future work can incorporate larger real-world datasets over extended periods of use and explore more diverse use cases to provide a more comprehensive understanding of the system's capabilities and limitations.}
% 
\rev{Third}, the interview participants live inside the United States, and only image descriptions written in English were collected and analyzed. Thus, this study may not reflect perspectives outside the United States or from non-English speaking contexts. Future research can explore the usage and limitations of LMM-based VQA systems across broader and diverse cultural backgrounds. 
% 
\rev{Fourth}, \bma{} cannot store conversation history. This limited functionality prevented users from sharing their ongoing interactions with the system. Thus, we were unable to fully understand users' prior experiences or analyze the data within broader contexts. 




%%%%%%%%%%%%%
\section{Conclusion}

This study investigates the application of LMMs, particularly through \bma, to enhance accessibility for PVI. Our research explores both the capabilities and limitations of the system by interviewing 14 visually impaired users and analyzing image descriptions generated by it. 
We identify significant limitations in \bma's context-aware and intent-oriented capabilities, including AI hallucinations, subjective interpretations in social and stylistic contexts, inaccurate recognition of people's identities, and inconsistent support in understanding and acting on user intentions. 
These challenges often lead users to rely on human assistance or personal strategies to compensate. 
Informed by these findings, we propose approaches to enhance interaction between PVI, \bma, and remote sighted assistants, emphasizing streamlined interactions, more accurate identity recognition, and reduced AI errors. We also highlight the potential of multi-agent systems, fostering collaboration among humans and AI, and suggest exploring AI-AI cooperation for tasks requiring specialized knowledge.


\begin{acks} 
We thank Samantha Paradero for her assistance in data collection.  
We also thank the anonymous reviewers for their insightful comments. 
This research was supported by the US National Institutes of Health, and the National Library of Medicine (R01 LM013330). 
\end{acks} 

==> sections/old_discussion.tex <==
\subsection{Task Offloading to \bma{} Through Distributed Cognition}


% [visual cognition, compare with bme, seeing ai, ocr, facebook ai, bring spatial awareness etc.]

% [human's own cognition process]

% [bme bringing another human's cognition, compare with bme], switch back and forth, hybrid, human+ai work together, two heads

% {\color{blue}
% [white cane vs bma]: real time vs pause, a tech problem, cannot replace white cane as o\&m skills
% }

% [hand off, when AI/human bring their knowledge, 
% fine tune the environment for individuals, how AI can analyze the environment better to understand the users' goal (360 panoramic view)]

% [understand the context, error state, e.g. remove eggshell rather than identify it; not just CV in seeing what is in the scene, but what to do]


%%%%%%%%%%%
% [bma's visual cognition]
% [human's own cognition process]
% bma is transition, human make it cog extension with adaptation, indication and opportunity that bma is a good start (thermostat, different prompts)
Our findings reveal that participants and \bma{} collaboratively work as interconnected components within the cognitive system, reflecting the principles of distributed cognition. Participants offload the burden of visual perception to \bma, enabling them to more effectively navigate and interact with their environment. This tool acts as a prosthetic for visual processing, transforming complex visual information into comprehensible audible text, which PVI can easily process. 


Unlike traditional prosthetics like the white cane, which extend PVI’s tactile senses, \bma{} is an active cognitive extension. It interprets visual data in real time, providing dynamic and creative assistance in various contexts. 
For example, it can read allergy-free labels on food packaging (Section~\ref{cooking}), identify colors and patterns for outfit matching (Section~\ref{fashion}), and describe scenes to enhance spatial awareness (Section~\ref{scene}). 
With its capability to interpret visual content in a detailed and accessible manner, \bma{} effectively simulates visual cognition for PVI.





% [individual adaptation:] how to accommodate challenges and limitations, tradeoff
% gap between what pvi expect and what they get 
Despite its advantages, \bma{} also presents several limitations and challenges.
To overcome these obstacles, participants have developed adaptive strategies.
They utilize their memory, inferential reasoning, and experiential knowledge alongside \bma{} to create a more robust cognitive extension within the distributed cognition system. 
For instance, when \bma{} recognized a thermostat but failed to give detailed information about how to adjust a thermostat, participants posed targeted questions to get more specific information or called for human assistance (Section~\ref{cooking}). 
In cases of AI hallucinations, participants rely on their spatial knowledge or seek human confirmation (Section~\ref{scene}). These adaptations illustrate the dynamic nature in distributed cognition, where participants actively reshape their interactions with technology to enhance cognitive support.
% 
% These instances indicate that opportunity that \bma is not perfect but a good start [related to distributed cognition]


% Moreover, participants creatively adapt \bma's visual interpretation capabilities to their intent in more creative and personalized contexts. 
Furthermore, participants creatively adapt \bma's visual interpretation capabilities to their personal needs and contexts. For instance, they combine \bma's outputs with their O\&M skills to enhance navigation (Section~\ref{navigation}) and supplement \bma's visual cues with their auditory, tactile, and olfactory senses to ensure safety when interacting with horses (Section~\ref{animal}). 
Participants also adjust their use of \bma{} when assessing fashion choices (Section~\ref{fashion}) or interpreting a pet’s expressions (Section~\ref{animal}).

These examples demonstrate how users actively shape their cognitive support systems, reinforcing the idea that distributed cognition is a dynamic process. By harnessing their own cognitive strengths and adjusting their interaction patterns with \bma, participants create a more flexible and robust approach to accessing visual information. 



% bma is transition, human make it cog extension with adaptation, indication and opportunity that bma is a good start (thermostat, different prompts)


% [artifact] address the need for visual input, how people can simulate bma's capability to visual cognition, simulation of bma in dcog system

% bma simulates pvi's visual cognition in dcog system



%%%%%%%% compared with white cane 
% Compared with white cane, 
% prosthetic are taking the visual load, managing it in alternative way, new prosthetic do it in another way different from white cane, bma is more dynamic, expensive, creative


% cane: extension of hand, limited, bma can extend it to far-away objects, both prosthetic

% o\&m skills in navigation, tactile information

%%%%%%%%%%%%%%%%%%%
% compare with ai-powered vqa
% seeing ai, ocr-based, facebook ai, bring spatial awareness etc, cannot provide conversations
% bma is external memory


\paragraph{Comparison with Non-LMM AI-Powered Systems}


Compared to non-LMM AI-powered systems like Seeing AI~\cite{SeeingAI2020} and Facebook AI, participants noted that \bma{} can process both graphic elements and text, offering more comprehensive and vivid interpretations of visual content (Section~\ref{cooking}). This capability enhances the distributed cognition system by incorporating a form of visual cognition that is superior to conventional systems.


Additionally, \bma{} facilitates interactive conversations with its users, a functionality absent in OCR-based visual interpretation systems. This conversational ability introduces an interactive cognitive process, where \bma{} not only decodes visual information but also engages in a dialogic interaction. This interaction enhances cognitive engagement, allowing users to clarify, question, and explore visual content in a more dynamic manner. 





% compare with human-assisted vqa
% [bme bringing another human's cognition, compare with bme], switch back and forth, hybrid, human+ai work together, two heads, helpful to get from diverse thoughts
% bma is NOT perfect but can provide some subjective info 

% aira - domain expert objective, bma (domain expert -- visual graphics) is playing more roles rather than giving visual description (fashion) 
% human is varied, not consistent, simulate human's conversation 

\paragraph{Comparison with Human-Assisted VQA Systems}
In human-assisted VQA systems, another human’s cognition is involved to support PVI. In these systems, participants offload visual processing and some aspects of reasoning to human assistants. 
For instance, human assistants can identify the colors of outfits; however, their capability may be limited by factors such as colorblindness (Section~\ref{fashion}) or they may get overwhelmed by an abundance of visual elements and overlook critical details (Sections~\ref{scene} and \ref{physical}). Moreover, services like Aira instruct their human assistants to provide only objective information~\cite{lee2020emerging,xie2023two}, which may limit the depth of cognitive support provided. 

In contrast, \bma{} offers consistent visual interpretations and goes beyond mere description by incorporating subjective judgments, like fashion suggestions. 
This capability allows \bma{} to not only support basic visual tasks but also integrate contextual understanding into its interactions. 
%
By doing so, \bma{} functions as an extension of the PVI's cognitive processes, adapting to various contexts and individual needs in ways that human assistants may not. Such a system enriches the distributed cognition framework by providing a more adaptive cognitive agent. This adaptability enables PVI to engage with their environments more seamlessly. 



% summary, bma as domain exeprt, subjective...



%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%resonate with goal

%break-down

% https://dl.acm.org/doi/abs/10.1145/3563657.3595977

% Our findings highlight the role of distributed cognition in the interaction between PVI and AI-powered assistive technologies like \bma{}. The distributed cognition framework, which views cognitive processes as interactions among individuals, artifacts, and socio-cultural elements \cite{hutchins1995cognition, hollan2000distributed}, provides a valuable lens for understanding how PVI adapt to and integrate these technologies into their daily lives.

% \subsubsection{Enhancing Spatial Awareness and Social Navigation}
% One of the key findings of our study is that AI-powered assistive technologies like \bma{} can significantly enhance PVI's spatial awareness and ability to navigate complex social situations. By providing detailed scene descriptions, these technologies often reveal spatial details that are not initially apparent to PVI, allowing them to gain a better understanding of their surroundings and social contexts.

% PVI can leverage this enhanced spatial awareness to assess and align with social norms, such as determining the appropriate attire for a given event or ensuring that their appearance matches that of their peers. This aligns with the distributed cognition framework's emphasis on the coordination between internal and external representations \cite{rogers2022hci, hollan2000distributed} and highlights the importance of designing assistive technologies that support users' sense-making processes in social situations.

% \subsubsection{Offloading Cognitive Tasks and Enhancing Engagement}
% Our findings also demonstrate how AI-powered assistive technologies can act as cognitive extensions for PVI, enabling them to offload cognitive tasks and enhance their engagement in various activities. In parenting roles, for example, PVI can use these technologies to describe and verify the appearance of their children, focusing on attributes like hair texture, skin complexion, and clothing styles and colors. This allows them to make informed decisions about their children's appearance and engage more meaningfully in family activities, such as reading books or participating in puzzles.

% By offloading the cognitive load associated with visual distinction, AI-powered assistive technologies enable PVI to participate more fully in family activities and social interactions. However, our findings also highlight the limitations of these technologies in providing goal-oriented information, underscoring the need for designers to consider the appropriate level of detail and context-awareness when developing assistive technologies for PVI.

% \subsubsection{Transforming Social Interactions}
% The detailed visual interpretation capabilities of AI-powered assistive technologies can also enable PVI to engage in more meaningful and authentic social interactions. By providing access to visual details that might otherwise be overlooked or taken for granted by sighted individuals, these technologies allow PVI to personalize their interactions and contribute more fully to social activities.

% For example, PVI can use these technologies to ensure that gifts are appropriately prepared and presented, or to read and respond to personal messages in a more genuine and emotionally resonant manner. Moreover, AI-powered assistive technologies can facilitate decision-making and autonomy within physical social engagement, allowing PVI to make informed choices based on the same visual information available to sighted individuals.

% These findings demonstrate how AI-powered assistive technologies can enhance PVI's social interactions by providing detailed visual interpretations and enabling them to perform tasks independently, fostering more genuine and joyful connections with others. This aligns with previous research that has explored how people utilize external cognitive resources to tackle complex challenges and facilitate communication and coordination within a distributed cognitive framework \cite{halverson2002activity, baumer2011comparing, wu2008collaborating, rogers2006distributed, perry2003distributed}.

% \subsubsection{Balancing AI Interpretations with Subjective Inputs}

% While AI-powered assistive technologies provide valuable information in various contexts, our findings show that PVI often adapt the outputs of these technologies to align with their own perceptions and combine them with other sensory information to ensure accuracy and safety.

% PVI may emphasize personal judgment over the subjective interpretations provided by these technologies, preferring the flexibility to override assumptions or integrate AI-based interpretations with their own sensory inputs. This strategy allows PVI to maintain a sense of control and autonomy in their interactions with the world, while still benefiting from the insights provided by AI-powered assistive technologies.

% These findings highlight the importance of designing AI-powered assistive technologies that allow for user customization and adaptability, enabling PVI to tailor the distribution of cognitive tasks to their individual requirements and abilities, and to balance AI interpretations with their subjective inputs.






% \subsection{Exploring Motivations for \bma{} Usage through Self-Determination Theory}
% % SDT: why participants use bma, why does it matter for the theory, SDT looks into pvi's use of assistive technology (fulfill user's needs) 

% % competence > tools + skills > BeMyAI is a great tool; it increases competence, which boost their confidence to be independent. Independence/agency/dignity is the primary reason blind people use assistive technology

% % sooyeon's independence paper

% Based on our findings, we identified several aspects that reflect the underlying motivations for using \bma{} and align with the principles of SDT. These aspects illustrate how \bma{} meets participants' psychological needs for autonomy, competence, and relatedness, which are crucial for fostering motivation and psychological well-being.


% % autonomy
% \textit{As for autonomy,} we found that \bma{} does not override the users' ability to apply their own judgment, instead granting them control over personal choices. Rather than making decisions for them, \bma{} provides users with the information needed to make informed choices.
% For example, participants preferred to rely on their own judgment over AI's suggestions for outfit matching (Section~\ref{fashion}). Similarly, P5 valued \bma’s ability to interpret her pet's status but chose to adapt the AI-generated information to fit her perceptions (Section~\ref{animal}).
% These instances emphasize that while \bma{} enhances autonomy by providing visual interpretations, it also supports users' autonomy to retain control over their personal decision-making.


% Furthermore, \bma{} boosts the autonomy of its users by addressing navigational needs. The tool proves effective in aiding localization and orientation, essential for PVI's independence. Participants demonstrated how \bma{} assists in navigation tasks by reading signages and identifying surroundings (Section~\ref{navigation}). 
% % 
% This capability enables users to navigate more independently without relying on constant human assistance. As a result, they gain more confidence and control over their environment, emphasizing the tool's role in enhancing autonomy.


% % competence
% \textit{As for competence,} \bma{} increases PVI's competence by providing them access to complex visual content that would otherwise be inaccessible. This tool interprets and transforms intricate visual data into accessible, audible text, allowing users to engage in various contexts of their daily lives. 
% %
% \bma{} has helped participants understand detailed graphics on food packaging, enabling safer dietary choices (Section~\ref{cooking}). 
% % 
% It has also provided descriptions of objects and bystanders, enriching environmental interactions and spatial awareness (Section~\ref{scene}). 
% % 
% Additionally, \bma{} has conveyed visual and textual details on Christmas cards, facilitating more genuine social exchanges (Section~\ref{physical}). 
% % 
% By converting visual information into formats that are usable for PVI, \bma{} supports and improves their ability to perform tasks competently. 


% % relatedness
% \textit{As for relatedness,} \bma{} enhances relatedness for PVI by enabling richer social interactions in digital, physical, familial, and human-animal contexts. In the digital realm, \bma{} helps users describe images, check image quality, and generate alt text, making them both recipients and active contributors of visual content on social media (Section~\ref{digital}). 
% % This functionality boosts their confidence and elevates their social media engagement.
% % 
% \bma{} facilitates communication between blind and sighted individuals by providing accurate visual descriptions, reducing the need for sighted people to perfectly describe images (Section~\ref{digital}). 
% % 
% In familial settings, it supports parenting roles (e.g., dressing their children) and family activities (e.g., puzzle assembling) (Section~\ref{physical}). 
% % 
% Additionally, \bma{} enhances interactions with animals, allowing for a deeper understanding and safer engagement by identifying their positions and behaviors accurately (Section~\ref{animal}). 
% % 
% In each of these scenarios, \bma{} not only supports but also amplifies the social, familial, and human-animal connectivity of users, demonstrating its profound impact on fostering relatedness within and beyond the visually impaired community.

% \vspace{3mm}

% % conclusion


% In this study, we have demonstrated how \bma{} aligns with the principles of SDT by enhancing autonomy, competence, and relatedness among users with visual impairments. Traditionally, SDT has been applied within the domains of gaming -- focusing on fun~\cite{deterding2016contextual,johnson2015all,ryan2006motivational,aufheimer2023examination}, and health -- emphasizing wellness~\cite{eilert2020osteoarthritis,guldenpfennig2019autonomy,muriana2021affecting}, in HCI research. We extend SDT by applying it to under-investigated areas, specifically safety and engagement within accessibility.

% \bma{} contributes to user safety by providing environmental descriptions that inform navigational risks like objects and bystanders (Section~\ref{scene}), increasing users' self-reliance and ability to navigate securely. In human-animal interactions, \bma{} offers critical visual interpretations like positions and directions of horses, which helps ascertain safety-related aspects and avoid dangerous situations (Section~\ref{animal}).


% Regarding engagement, \bma{} enriches participant interactions across digital, physical, and familial contexts (Section~\ref{digital} and~\ref{physical}). It bolsters social engagement by facilitating accurate communication of visual content, thereby making digital platforms more accessible and enjoyable. In familial settings, it supports essential activities, enhancing the quality of interactions and shared experiences. 

% These enhancements across the domains of safety and engagement not only fulfill the immediate functional needs of users but also profoundly contribute to their psychological needs for competence, autonomy, and relatedness as outlined by SDT. By addressing these crucial areas, this study broadens the scope of SDT, showing its relevance and utility in improving accessibility in technology use.

==> sections/old_findings.tex <==
% \subsection{\textcolor{red}{Distributed Cognition}}
% % artifacts are objects or tools that individuals use to support or extend their cognitive processes. 


% % Distributed cognition is a theoretical approach that is concerned with the interactions among people, artifacts, and both internal and external representations. Rather than focusing exclusively on an individual's internal cognitive processes, that traditional cognitive approaches do, it focuses on the processes that take place in an extended ‘cognitive system’. These include verbal and non-verbal behavior, the coordinating mechanisms used by social actors, the forms of communication that take place, and the way tacit and explicit knowledge is shared and accessed. One major benefit is the explication of the complex interdependencies among people, artifacts, and technological systems that often can be overlooked when using traditional theories of cognition. (Rogers)

% Distributed cognition is a framework that conceptualizes cognitive processes not as confined within an individual's mind, but rather as interactions among individuals, artifacts, and socio-cultural elements~\cite{hutchins1995cognition}.
% % 
% In this framework, a cognitive process is defined by the functional relationships among the elements that participate in it, rather than by their spatial colocation~\cite{hollan2000distributed}. Furthermore, cognitive processes often require coordination between internal and external representations~\cite{rogers2022hci,hollan2000distributed} and can be distributed across time~\cite{hollan2000distributed}.



% Research in HCI has explored the application of distributed cognition in explaining how people utilize external cognitive resources, like artifacts and environmental elements, to tackle complex challenges~\cite{halverson2002activity,baumer2011comparing}. 
% % 
% For example, Wu et al.~\cite{wu2008collaborating} investigated how families dealing with memory impairments collaborate on everyday tasks, examining the mechanisms for accessing and sharing knowledge~\cite{rogers2006distributed}, facilitating communication and coordination within distributed cognitive framework~\cite{perry2003distributed}. 
% % 
% Nobarany et al.~\cite{nobarany2012facilitating} applied this framework to explore how analysts, reasoning artifacts, and user interface elements contribute to supporting unanticipated reuse in distributed collaboration. 
% % 
% In this study, we examine how PVI off-load cognitive efforts such as visual, remembering, and reasoning onto artifacts like \bma{} to achieve their goals. Additionally, we explore how these artifacts support and extend PVI's cognitive processes in their daily activities. 

% {\color{red}
% offload visual perception (missing) to be my ai]
% prosthetic are taking the visual load, managing it in alternative way, new prosthetic do it in another way different from white cane, bma is more dynamic, expensive, creative

% gap between what pvi expect and what they get

% cane: extension of hand, limited, bma can extend it to far-away objects, both prosthetic

% [artifact] address the need for visual input, how people can simulate bma's capability to visual cognition, simulation of bma in dcog system

% bma simulates pvi's visual cognition in dcog system


% [individual adaptation: ] how to accommodate challenges and limitations, tradeoff


% interchangably work together, two entities 
% }



% \subsection{Self-Determination Theory}
% Self-Determination Theory (SDT) is a psychological framework for understanding human intrinsic motivation~\cite{deci1985intrinsic}.
% % 
% At its core, SDT posits that people are inherently motivated to pursue personal growth and fulfillment, driven by three fundamental psychological needs: autonomy, competence, and relatedness.
% % 
% These needs are defined as follows: autonomy involves control over one’s own actions; competence refers to the capability of doing something; and relatedness pertains to forming meaningful connections with others.
% % 
% SDT argues that fostering conditions that support these psychological needs, such as participation in activities that resonate with personal values and interests, eventually cultivates the most volitional and highest quality forms of intrinsic motivation~\cite{deci1985intrinsic,deci2000and,ryan2000self}.



% In recent years, HCI field has increasingly adopted SDT as a framework in its research endeavors~\cite{deterding2016contextual,johnson2015all,ryan2006motivational,aufheimer2023examination,eilert2020osteoarthritis,guldenpfennig2019autonomy,muriana2021affecting,ford2012self,huang2019investigation}. 
% Predominantly, these studies have concentrated on the domains of gaming and gamification~\cite{deterding2016contextual,johnson2015all,ryan2006motivational,aufheimer2023examination}, 
% health and well-being~\cite{eilert2020osteoarthritis,guldenpfennig2019autonomy,muriana2021affecting} and education~\cite{ford2012self,huang2019investigation}.
% % 
% The application of SDT enables HCI researchers to examine these domains through the lens of psychological needs, offering deeper insights into the motivations that drive user engagement.
% % 
% In this study, we analyze the motivations of PVI for using \bma{} in their daily lives. We aim to extend SDT framework, traditionally applied within the domains of gaming (emphasizing fun) and health (emphasizing wellness) in HCI research, to explore its applicability to the under-investigated areas of safety and engagement within accessibility. 







\section{OLD Findings [will be removed]}
\label{sec:findings}


Seven participants (P1, P6-8, P10, P12, P14) highlighted their use of \bma{} for reading tasks, which is a prevalent need within VQA systems~\cite{avila2016remote,lee2020emerging,BME_100ways}. Their activities spanned reading mail, newspapers, and labels. 
% 
In this section, however, we aim to explore beyond basic reading functions, which are already well-addressed by existing technologies like OCR, to examine the more emerging and interactive practices introduced by LMM technologies. Specifically, we delve into how \bma{} supports managing personal and household tasks, understanding spatial environments, and engaging in social interactions. 

Our analysis reveals that \bma{} is part of the cognitive system in these contexts. In each use case, we examine how participants offload their cognition to \bma{} in \textit{``Artifact as Cognitive Support''}, as well as understand how participants accommodate challenges and limitations associated with \bma{} and how they creatively adapt \bma's capabilities to more creative and personalized use cases in \textit{``Individual Adaptation and Cognitive Strategies.''}




% [more than visual cog, understand some tasks, help in decision-making]

% why we use ``artifact as cognitive extension'' and ``Individual Adaptation and Cognitive Strategies''

% connect to contributions to the paper

% offload, assimilation?, reconfigure, accommodation (how we change what we do)

% the tool is part of the cognition

\subsection{Managing Personal and Household Tasks}
% Seven participants (P1, P6-8, P10, P12, P14) highlighted their use of \bma{} for reading tasks, which is a prevalent need within VQA systems~\cite{avila2016remote,lee2020emerging,BME_100ways}. Their activities spanned reading mail, newspapers, and labels. 
% % 
% In this section, however, we aim to explore beyond basic reading functions to examine the more complex and interactive tasks that participants engage in with \bma. Specifically, we will investigate how \bma{} is utilized in managing household appliances, assisting with cooking and dining, and providing fashion-related help.



%%%%%%


% It gives me the confidence I need to know that I can because like for instance, when I don't know the directions, I can just you know have it scan the box and then you know the directions will be written and then I'll know exactly what the directions say, so I can you know cook the product in the right amount of QuickTime. (P7, cooking and dining)


In this section, we explore how \bma{} facilitates participants in daily home activities, including using household appliances, cooking and dining, and fashion help. It highlights how \bma{} improves the practical aspects of home and personal life.  


\subsubsection{Help with Household Appliances}
\label{appliances}
Participants engaged \bma{} for assistance with household appliances, categorically divided into grid keypad and rotary control appliances. These devices necessitate tactile interaction for operational inputs, requiring actions such as pressing buttons or turning dials for setting controls or making selections. 
% 
% In facilitating these tasks, \bma{} functions by elucidating visual content. Participants take actions to align \bma's capabilities with their intent (e.g., ask specific questions relative to the visual content), or seeking alternative means (e.g., calling human volunteers) to fulfill their goals.



% layout 1: keypad panel with columns and rows, such as keypad, microwave. (description: P11) 
% 2, 5, 9, 11, 14
% layout 2: dail need rotating actions, such as thermostat, washer
% P1, P2, 4, 5, 13, 14

% \paragraph{\textbf{Environment:}}
% This use case primarily occurs within home settings (P1, P2, P9, P11), extending to scenarios involving travel (P4, P13, P14) or transitioning to new living spaces (P5). 

% [users know the environment better than AI]

% \textcolor{red}{[bma has limitations, but the users make it creatively as cognitive extension by overcoming its limitations]}


% \newtcolorbox{mybox}{colback=blue!5!white,colframe = blue!75!black}
\begin{mybox}
The picture shows the control panel of a GE washer/dryer. There are three main controls visible:\\
- On the left, there is a knob for Load Size with options Small, Medium, and Large.\\
- In the center, there is the GE logo and below it, the words ``WASHER / DRYER'' and a Start button.\\
- On the right, there are two knobs. The top knob is for Dryer Cycles with settings for Cottons (Less Dry, Optimum Dry, More Dry), and Delicates. The bottom knob is for Washer Cycles with settings for Quick Rinse, Spin, and various wash times (10, 6, 4, 2 minutes).\\
The Start button is a round, black button located below the GE logo and the words ``WASHER / DRYER''.
\end{mybox}
\captionof{figure}{Image description of a control panel provided by P14.}


\paragraph{Artifact as Cognitive Support:}

% \textcolor{red}{[Artifact as Simulation of Visual Cognition?]}

Five participants (P2, P5, P9, P11, P14) utilized \bma{} to navigate the grid layout of keypad panels on appliances, characterized by organized rows and columns. 
% 
\bma{} reduces participants' cognitive load of visually searching the layout by providing structured verbal descriptions.
% 
For example, in detailing a microwave's control panel, \bma{} begins by identifying the number of rows and columns, followed by employing directional (e.g., top, bottom, left, right, center) and sequential (e.g., second row, from left to right) terminology to guide users through the panel's arrangement. 

% [discussion:] This interaction reduces the cognitive effort required by participants to navigate unfamiliar control panels, effectively integrating into their cognitive system. 


% \begin{quote}
%     \textit{``Like the control panel of my microwave, it would tell me there are five rows of buttons. The buttons that are arranged in three columns. The top left button is start, the top middle is cook time, the top right is defrost, and then it would go down to the rows of buttons and give me similar descriptions for each one.''}  (P11)
% \end{quote}


%%%%%
However, we also identify limitations in the \bma’s ability to support all cognitive needs effectively in helping with household appliances. Six participants noted its inadequacy in accurately describing rotary control appliances like washers (P1) and thermostats (P2, P4, P5, P13, P14). These appliances require \bma{} to interpret current settings as users adjust dials for time, mode, or temperature. 


Critically, participants observed that \bma{} lacks a goal-oriented approach, often offering broad descriptions of visual elements without honing in on the user's specific objectives. P12 highlighted this issue, remarking, \textit{``Be My AI loves to make general descriptions, and it doesn't know what to focus on,''} leading to user frustration. For example, while \bma{} recognized a thermostat on the wall, it failed to convey essential details such as the current temperature setting or instructions for temperature adjustment. 

% [discussion:] not interpret distributed cognition, move to discussion, not use too much DCog: This reveals gaps in the cognitive system where the tool does not fully align with the user's cognitive goals, necessitating additional cognitive effort from users to compensate for these shortcomings.}



\paragraph{Individual Adaptation and Cognitive Strategies:}
To overcome these limitations, participants developed adaptive strategies. For example, P5 posed targeted questions to \bma, such as \textit{``What is the arrow pointed at right now on the current setting?''} This approach refined \bma's output to be more precise and relevant to the setting, enabling P5 to adjust the dial accurately.
% 
P12, on the other hand, aimed to improve \bma's focus by carefully aligning the camera with the specific item of interest, thus directing \bma{} to concentrate on particular elements rather than offering broad, scene-wide descriptions.
% 
These adaptations indicate how users actively reshape their interactions to optimize cognitive support. 

% [discussion:] These adaptations are indicative of the dynamic nature of distributed cognition, where users actively reshape their interaction patterns to optimize cognitive support. 


Additionally, eight participants (P1-3, P7, P8, P12-14) compared \bma{} with video-based human-assisted VQA systems, noting that the latter offers more adaptive and contextually aware support in tasks that require continuous real-time feedback, such as dial adjustments.
P13 shared an instance where volunteers from \bme{} understand her intent beyond mere identification of objects like a thermostat.
% 
Volunteers can provide immediate, actionable feedback and guidance, facilitating a more effective interaction through conversation.


\begin{quote}
    \textit{``I ended up pulling up a volunteer, and the volunteer was fantastic. He goes, `You know, these are tricky.' And he says, `It looks like it's set at 69. What do you want?' And I said, `71.' He goes, `Turn it, turn it. Yep, it's 71 from what I can tell.' And I went, `Cool.'''} (P13)
\end{quote}


In summary, \bma{} reduces the visual load involved in using household appliances, but it is not goal-oriented. Participants adapt \bma's capabilities to their intent by asking specific questions about the visual content or by seeking alternative means, such as calling human volunteers, to fulfill their goals.


%%%%%%%%%%%%%%
\subsubsection{Cooking and Dining}
\label{cooking}
Participants leveraged \bma{} for various culinary tasks, including identifying specific foods among similar items, like drink cans (P6), coffee beans (P7), cans of tomatoes or avocados (P10), chili spices (P10), and Campbell's soup cans (P13). They also used it to access cooking instructions regarding time and temperature (P7, P8, P9), read non-Braille recipe books (P9), and identify ingredients and suggest recipe (P12).
% 
% In these tasks, \bma{} converts graphical content to audible formats and offers recipe recommendations. Participants use \bma{} as a cognitive aid in accessing visual information and navigating the detailed recipes it provides. 



% \paragraph{\textbf{Interaction with the Environment:}}
% In many cognitive tasks, individuals rely on the knowledge and skills of others within their environment. 

% This use case typically happens in pantries (P2), kitchens (P5-10, P12, P13), and during shopping trips (P10). 
% % 
% The environmental context significantly influences the effectiveness of \bma. For instance, P5 reported challenges related to excessive or inadequate lighting, which hindered the \bma's ability to interpret visual cues. 
% In response to these conditions, \bma{} advises on retaking pictures for better clarity, exemplifying cognitive artifacts adapt to environmental limitations. This highlights a dynamic interaction where both the user and the artifact adjust behaviors to optimize performance. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{images/cooking - eggshell.png}
\caption{Image description of eggs in a frying pan, followed by a question to check for the presence of eggshells. Example was originally drawn from X (\url{https://x.com/BeMyEyes/status/1706335189985526191})}
\end{figure}


%%%%%%%%
\paragraph{Artifact as Cognitive Support:}

\bma{} transforms complex visual information, such as graphics on food packaging, into comprehensible audible text that PVI can process. It acts as a cognitive proxy, interpreting and relaying information that would otherwise be inaccessible, thus reducing participants' cognitive load associated with tasks such as identifying specific food items or following cooking instructions.


Unlike other AI-powered VQA systems like Seeing AI and OCR, \bma{} processes graphic elements in addition to text. 
% 
For example, \bma{} informed P2 about an \textit{``allergy information emblem''} on product packaging, aiding in selecting allergy-safe foods. \bma{} detailed not just the brand name but also specific allergy-free labels that indicated the absence of common allergens like gluten, dairy, and sesame.  


% Participants noted that \bma{} surpasses other tools like Seeing AI and OCR in delivering visual-related insights. While Seeing AI and OCR excel in text extraction from items, identifying canned or boxed items swiftly through their quick read feature, \bma{} extends its capabilities to interpreting graphic elements, such as logos. 



Moreover, \bma{} enhances the cooking and dining experience through its ``ask more'' function, which allows participants to interactively engage with the artifact to receive tailored cooking advice. P12 utilized this feature, who sought recipe suggestions by inputting available ingredients: \textit{``I typed in the chat that I have chicken, pasta sauce, onion... and I asked for \bma, you know, to provide a recipe.''}
% 
% \begin{quote}
%     \textit{``The way I approached this was, I typed in the chat, that I said that I have a chicken, pasta sauce, onion, and I think one or two other things, and I asked for Be My AI, you know, to provide a recipe.''} (P12)
% \end{quote}
% % 
Responding to P12's input, \bma{} offered practical cooking instructions that included a list of ingredients, preparation methods (e.g., boiling, dicing, cutting into bite-sized pieces), required cookware, steps detailed with timing and sequencing, and seasoning tips.

% , demonstrating its ability to contribute beyond basic recognition and description tasks. 



% The environmental context significantly influences the effectiveness of \bma. For instance, P5 reported challenges related to excessive or inadequate lighting, which hindered the \bma's ability to interpret visual cues. 
% In response to these conditions, \bma{} advises on retaking pictures for better clarity, exemplifying cognitive artifacts adapt to environmental limitations. This highlights a dynamic interaction where both the user and the artifact adjust behaviors to optimize performance. 




\paragraph{Individual Adaptation and Cognitive Strategies:}
% users' cognitive, memory, perception or action. 


Participants employed specific strategies to manage the cognitive load involved in cooking tasks. By leveraging \bma{} as an external memory aid, P12 accessed complex cooking instructions in a step-by-step manner, reducing the need to retain and remember extensive procedural details from cookbooks or websites. 
% 
% Despite the support from \bma, P12 encountered challenges with the volume of information provided by \bma, noting, \textit{``it is a lot to, kind of, keep in your mind.''} 
% % 
% This led to a repetitive cycle where P12 listened to recipes, executed one or two steps, and then revisited the recipes for subsequent procedure. 
% 
This interaction with \bma{} involved retrieving information, processing it, and then executing based on the guidance received, illustrating the dynamics between P12's cognitive processes and the use of the artifact. 
% While \bma{} significantly reduces the need to consult external sources, it also necessitates repeated engagement to manage detailed tasks effectively. 
% Consequently, P12 was able to adaptively navigate the complexities of cooking, effectively utilizing \bma's support to address the cognitive challenges posed by detailed culinary tasks. 



In summary, \bma{} converts the graphical content on food packing to audible formats and offers recipe recommendations for cooking and dining. Participants use \bma{} as a cognitive aid in accessing visual information and navigating the detailed recipes it provides. 


%%%%%%%%%%%%
\subsubsection{Fashion Help}
\label{fashion}
\bma{} has served as a valuable tool for fashion-related tasks, assisting participants in several key areas: identifying colors of clothes (P2, P7, P9, P13), detailing patterns or designs on clothes (P2, P9), offering suggestions for assembling stylistically harmonious and color-coordinated ensembles like outfits, shoes, and jewelry (P2, P4, P5, P6, P12), and checking makeup (P5, P10).
% 
% In these tasks, \bma{} enhances decision-making in fashion by offering precise color identification and tailored fashion suggestions. Participants respond diversely to these capabilities. Some embrace the suggestions, finding that they bolster confidence and assist in assembling outfits, while others prefer to rely on their own judgment and decision-making to coordinate their attire.






% \paragraph{\textbf{Environment:}}
% This use case predominantly unfolds within the home setting, where participants select clothing, accessories, and apply makeup to prepare for work, social activities, or daily outings. 

% align ties with shirts
% So I picked that one because I knew what color it was. And I hung that shirt on my closet. And then what I did was I hung 4 different ties that I had, but I hung them over the shirt so that way Be My AI could see how it looked on the shirt. And after taking the picture of those things, I had a conversation with Be My AI. The first thing I said was basically, which ties goes well with the shirt. And it said that I should wear the black tie. it's a good option for basically any setting. (P12)




\begin{mybox}
The picture shows a light blue, long-sleeved dress shirt hanging on a black hanger. There are three ties hanging on the right side of the shirt. From left to right, the first tie is navy blue with small white paisley patterns, the second tie is solid red, and the third is solid black. The shirt is labeled ``Stafford'' and is size XL. The shirt is hanging on a wooden door, and there are some items on a shelf above the door, including a box of Nature Valley granola bars and a box of Mini Wheats cereal. To the left of the shirt, there is a partial view of a black office chair with a grey towel and a brown blanket on it.\\
Follow-up Question: Which tie should I wear with the shirt?\\
The solid black tie would be the most classic and versatile choice to wear with the light blue dress shirt. It creates a sharp contrast and is suitable for most formal occasions.
\end{mybox}
\captionof{figure}{Image description of a shirt with three ties and follow-up question on which tie to wear, provided by P12.}



\paragraph{Artifact as Cognitive Support:}

Participants have found \bma{} exceptionally precise in taking the visual load by identifying colors and patterns on clothing, as well as in assessing makeup, with no discrepancies reported. For instance, P5 effectively used \bma{} to verify the color, placement, and overall balance of her makeup, ensuring there were no mismatches or issues. 



This accuracy is particularly valued in fashion-related tasks, where \bma{} demonstrates a more consistent and reliable perception of color compared to human assistance. 
P4 pointed out that human assistants, such as \bme{} volunteers, often have subjective interpretations, stating, \textit{``each volunteer has a different way of seeing things''}. 
% 
P9 echoed that \bma{} maintains consistent detail in its interpretations, whereas human volunteers can vary significantly in their visual descriptions: \textit{``Sometimes they might not understand exactly, or like how much you want it to be described; they don't tell you the same description.''}



P12's experience further underscores the reliability of \bma{} over human volunteers in color identification. He shared an instance where a colorblind volunteer, without disclosing the colorblindness, provided incorrect color information of a tie. 
This example underscores \bma's utility as a reliable tool for accurate color matching, essential for appropriate fashion decisions, as P12 mentioned: \textit{``This is a really good application for \bma{} because you don't have to rely on someone's color vision.''}


% indepdence -- you don't have to rely on someone's color vision


Moreover, \bma{} enhances decision-making in fashion by providing suggestions to create stylistically coordinated outfits. P9 consulted \bma{} to harmonize colors of a top and dressy pants effectively, and P12 used it to select a tie that complemented his shirt. 
% 
A notable example is P2's use of the ``ask more'' function to complete a fall-season look with a turquoise top.  
Concerned about the seasonality of a turquoise top, P2 asked \bma, \textit{``Is this too summery of a color? Could I wear it in the fall?''} \bma{} suggested, \textit{``Turquoise is typically a bright color that's considered more of a summer-spring color, but you could tone it down into more of a fall look with a cardigan or chunky boots.''} Following this advice, P2 selected a grayish taupe pair of ankle boots, and upon capturing their image, \bma{} confirmed, \textit{``This might pair well with the turquoise top to make it more fall appropriate.''}







\paragraph{Individual Adaptation and Cognitive Strategies:}

% confidence -- know the outfits are matching


Participants were divided regarding \bma's fashion suggestion functionality. Some appreciated this feature because it \textit{``definitely creates more confidence''} (P2) in preparing outfits for specific occasions, such as work or sports events. For instance, P5 found \bma{} helpful to \textit{``lay out [her] outfit before the race,''} enhancing her preparation and confidence for race day. 



However, other participants (P6, P7) held the opposite views. 
While they utilized \bma{} to obtain descriptions of colors and patterns, they hesitated to rely on its fashion suggestion. These participants preferred to make their own judgment and choices about outfit matching, emphasizing the importance of human subjectivity in fashion decisions. 
% 
P6 expressed concerns about the AI's ability to replicate human subjectivity, remarking, \textit{``It's interesting how AI is being taught to simulate kind of the human factor of things.''}
% 
She linked her skepticism to instances where AI-generated responses were \textit{``strange''} and \textit{``complete nonsense,''} which contrasted with human creativity and nuanced understanding. 



\begin{quote}
    \textit{``No, no, no, no, I would never use it to do anything that required human subjectivity... I just don't trust AI with a task that is supposed to be subjective like that, particularly visual like that. Have you ever seen AI weirdness?... I think that just goes to show why I'm not gonna trust AI with my fashion yet.''} (P6)
\end{quote}


% [discussion:] This divergence in user experience underscores the opportunities and challenges in designing AI-powered VQA systems that adequately simulate human-like decision-making processes in subjective domains, such as fashion.


In summary, \bma{} enhances decision-making in fashion by offering precise color identification and tailored fashion suggestions. Participants respond diversely to these capabilities. Some embrace the suggestions, finding that they bolster confidence and assist in assembling outfits, while others prefer to rely on their own judgment and decision-making to coordinate their attire.



%%%%%%%%%%%
%%%%%%%%%%%
\subsection{Understanding Spatial Environments}

In this section, we examine how \bma{} enhances spatial awareness through scene descriptions, locates dropped objects, and facilitates navigation. It highlights \bma's role in improving participants' ability to interact with and navigate their surroundings.



\subsubsection{Scene Description}
\label{scene}

Participants utilized \bma{} for detailed scene descriptions across both indoor environments, such as theaters (P2) and room layouts (P3, P7, P9, P13), and outdoor settings, including holiday decorations (P5) and street scenes (P11, P12). 
% 
% In these tasks, \bma{} acts as a cognitive extension by providing comprehensive scene descriptions that enhance participants' perception of their surroundings. 
% Participants improve spatial awareness with these descriptions, such as ensuring their attire aligns with others to boost confidence in concerts.


\begin{figure}[t!]
\centering
\includegraphics[width=0.8\textwidth]{images/scene description.png}
\caption{Image description of a soccer stadium. Example was originally drawn from X (\url{https://x.com/darren_keepers/status/1731118043898716371})}
\end{figure}


\paragraph{Artifact as Cognitive Support:}


Six participants (P2, P3, P7, P9, P13, P14) valued \bma's detailed scene descriptions for increasing their spatial awareness. 
It often reveals spatial details that are not initially apparent, as noted by P11, \textit{``It gives me unexpected information about things that I didn't even know were there.''} 
% 
\bma{} provides comprehensive visual information, augmenting participants' visual cognition by detailing objects by color, size, shape, and spatial orientation (e.g., ``on the left,'' ``to the right,'' ``in the middle,'' ``in the background''). It also describes dynamic elements like bystander actions (e.g., ``sitting''), text on signs or advertisements, and the overall atmosphere (e.g., ``peaceful and natural,'' ``cozy and cheerful holiday vibe,'' ``warm and inviting atmoshpere''). 


These detailed scene descriptions offers a richer sensory experience than those often provided by human assistants. Participants particularly appreciated \bma{} for its ability to handle visually-overloaded scenes with less subjectivity than human assistants. P2 pointed out that human assistants often feel overwhelmed by the abundance of visual elements, struggling to decide what to describe. 
% 
In these scenarios, human assistants prioritize and focus on elements they deem important and potentially overlook other details. In contrast, P9 highlighted that \bma{} does not ignore details that human assistants might consider unimportant. 

% highlighted \bma's comprehensive visual interpretations of scenes, as human assistants assume a priority and focus on particular things that they believe important, and ignore visual information they think unimportant.  

\begin{quote}
    \textit{``Maybe a family member wouldn't think that I would want to know that there was like a picture frame hanging in the wall or something... But \bma{} just described everything, so like, it is nice because you get to imagine how something really might look or how the house might be decorated or things like that.''} (P9)
\end{quote}


% AI hallucinations
Despite these advantages, there are notable drawbacks with \bma{} related to AI hallucinations, errors where the artifact inaccurately identifies objects that aren't present. 
% 
For instance, \bma{} erroneously added nonexistent details to scenes, such as an object mistakenly reported behind P3 and incorrect features in P5's home. 
% 


% [discussion:] These inaccuracies underscore the need for further refinement in AI-powered VQA systems, aiming to achieve an optimal balance between the comprehensiveness of scene descriptions and their precision, without overcompensating by adding excessive or incorrect details.




\paragraph{Individual Adaptation and Cognitive Strategies:}

% increase spatial awareness
% {\color{blue}
% \sout{Six participants (P2, P3, P7, P9, P13, P14) valued \bma's detailed scene descriptions for increasing their spatial awareness. 
% \bma{} often reveals spatial details that are not initially apparent, as noted by P11, \textit{``It gives me unexpected information about things that I didn't even know were there.''} }
% % 
% \sout{P2 exemplified the benefit of this scene awareness, who used \bma{} to gain a better understanding of social contexts that sighted individuals might perceive unconsciously. At a concert, P2 was concerned about her attire's misalignment with the crowd. She described her use of \bma{} to assess the audience's dress code:} 


% \begin{quote}
%    \textcolor{red}{remove:} \textit{``Like it told me, you know, like the men are mostly wearing button-ups and women are wearing dresses. Okay, cool. I wore a dress also. So I'm on par with everybody. So yeah, those kind of, I guess like contextual things that, you know, sighted people are just picking up incidentally without really having to think about it, you know, it can give you more access to that.''} (P2)
% \end{quote}
% }


% AI hallucinations: confirm with human assistant

To overcome issues with AI hallucinations, participants adopt various strategies to ensure accuracy in the visual information provided by \bma. For instance, P3 recounted an incident where \bma{} inaccurately reported an object behind her. To confirm this, P3 consulted a human assistant, who verified that there was indeed nothing behind her in the picture. 

On the other hand, P5 shared an experience where \bma{} added non-existent details to an image at her home, including elements supposedly alongside their dogs. Relying on her familiarity with the environment, P5 was able to identify these inaccuracies without external assistance. This reliance on personal knowledge illustrates how participants used their understanding of familiar surroundings to challenge and correct the AI's interpretations. 



% participants either consult human assistants for confirmation (P3) or rely on their existing knowledge to discern inaccuracies (P5). 


% ``so apparently the Be My AI said there was an object behind me and there really wasn't in the image description. So then when I went and asked somebody, you know what is behind me and they said there wasn't anything behind you in the picture.'' (P3)

% ``it was at my own house. I took a picture of something and it was with my dogs in the picture. And it like added a bunch of stuff to the picture. I can't even remember exactly but it added some details that weren't in my house.'' (P5)

% [discussion:] This adaptive approach demonstrates how participants integrate \bma{} into their cognitive and perceptual frameworks, using it alongside human input to navigate and interpret complex environments.




In summary, \bma{} acts as a cognitive extension by providing comprehensive scene descriptions that enhance participants' perception of their surroundings. Despite its efficacy, it is subject to the limitations of AI hallucinations. To overcome this issue, participants either consult human assistants for verification or rely on their own knowledge to pinpoint inaccuracies.

% Participants improve spatial awareness with these descriptions, such as ensuring their attire aligns with others to boost confidence in concerts.


%%%%%%%%%%%
\subsubsection{Locating Dropped Objects}
\label{locate_object}
The sequential descriptions provided by \bma{} assist participants in locating dropped objects (P4, P12, P13) such as earbuds and hair ties. 
% Participants enhance this functionality by integrating their auditory perception and spatial memory, enabling them to fine-tune the camera's positioning for more accurate scanning and help \bma{} concentrate on the relevant area. 



\paragraph{Artifact as Cognitive Support:}
Participants found that \bma's structured approach to describing surroundings aids in locating dropped objects. By systematically detailing the environment using a \textit{``top to bottom, left to right''} sequence, the artifact helps orient users more effectively compared to random starting points. 
% 
For example, \bma{} enhances spatial orientation by providing specific relative locations. After a general description of the scene, it indicates, \textit{``picture of a carpet with a hair tie in the upper right hand corner,''} (P13) or notes 
\textit{``the earphones are directly in front of you, between your feet''} (P12). 
These descriptions allow participants to pinpoint lost objects with greater accuracy.



\paragraph{Individual Adaptation and Cognitive Strategies:}

Participants utilized \bma{} by integrating it with their own sensory and cognitive strategies to locate dropped objects. They enhanced their use of the artifact by relying on auditory cues and spatial memory, which helped in initially estimating the dropped object's location. This approach allowed them to optimize the camera angle for taking pictures that \bma{} would analyze. 
For instance, P4 used his \textit{``listening skills''} to determine the location where the object fell and guided where to point the camera accordingly. 
% 
Similarly, P12 adjusted his position slightly backward from the seating area to capture a better overview of the floor where the earbuds were dropped. 
% 
These adaptions illustrate how participants combine their understanding of the environment with \bma's technological capabilities to manage tasks that require spatial awareness.


In summary, \bma's sequential descriptions support participants in finding dropped objects. Participants leveraged their auditory skills and spatial memory to adjust the camera's position, allowing for more precise scanning and enabling \bma{} to focus on the intended search area.




%%%%%%%%%%
\subsubsection{Navigation}
\label{navigation}
\bma{} is used for navigation tasks, such as localizing and orientating participants by reading airport signages (P2, P5), and store names when disoriented (P10). 
% 
% It boosts spatial awareness and independence, although some participants question its practicality and safety during navigation. However, there is consensus that \bma{} can only complement, rather than replace participants' orientation and mobility (O\&M) skills. 



\paragraph{Artifact as Cognitive Support:}

Participants (P2, P5, P10) employed \bma{} as a tool to assist in localization and orientation when approaching their destinations. 
It reduces the cognitive process by offloading visual tasks such as reading signages and recognizing surroundings.
% 
For instance, P2 utilized \bma{} to identify gate numbers at the airport, which helped her determine the location and navigate accordingly. 
% 
Likewise, P5 used \bma{} to read a signage indicating the direction to the transportation area at the airport, while P10 took pictures of her surroundings for orientation when lost in her neighborhood.  
% 
Such instances illustrate \bma's role in providing participants with \textit{``better spatial awareness of what's going on around [them]''} (P5), thereby allowing participants to gain \textit{``more independence and be more familiar with [their] environment''} (P10).
% These participants found the visual interpretations from \bma{} to be accurate and helpful in identifying when a picture was incomplete or blurry. P5 mentioned that \textit{``\bma{} will say that there were some words visible but not the whole sign so that you can take another picture. Or sometimes it will tell you that it's blurry so it contextually knows and it tells you when the information is incomplete.''} 

% 




However, other participants (P6, P11, P13, P14) reported challenges with \bma{} for navigation, particularly due to its limited camera view and the practical issues of mobility. 
As P6 described, participants \textit{``have to stand there and keep taking pictures and taking pictures,''} check what's captured, determine if it's helpful for navigation, and adjust the angle for another pictures. This iterative process can be time-consuming and might cause self-consciousness, as \textit{``taking constant pictures with their camera could also look weird''} (P6) to bystanders.


Moreover, P13 critiqued that \bma{} is not goal-oriented enough to aid navigation because of its broad descriptions. For instance, she used \bma{} to find a specific office, but it failed to read the office's door number and instead \textit{``It sa[id] something like `wall with door,' which is, you know, not particularly helpful.''}



% P13 indicated that \bma{} could be a good cognitive extension in navigation if identifying the exact door number, along with more information regarding the direction, distance. For instance, \textit{``it says you know, stairs in front and it's like, Okay, that's great, but where are they? How far are they? Are they going up? Are they going down? Is there a railing?''} (P13)




\paragraph{Individual Adaptation and Cognitive Strategies:}


In navigation, participants combined \bma's visual cognition with other sources of guidance. When using \bma, they often knew they were near their intended areas based on prior help from human assistants (P2, P5) or through their existing mental map (P10). For instance, after getting directions from a human assistant and was seated in the Gate 12 area, P2 leveraged \bma{} to move from Gate 12 to Gate 13. This demonstrates the integration of multiple sources of information.  


Despite the varied feedback on \bma, participants agreed that \bma{} is \textit{``not a replacement for [their] mobility skills or just any skills in general''} (P14). P5 elaborated that due to the limited information captured and interpreted by \bma, it can only provide partial navigational details, such as the presence of obstacles, noting \textit{``it's not gonna be able to tell you, like, to protect you every step of the way.''} 


Consequently, participants integrate \bma{} with their orientation and mobility (O\&M) skills to enhance their navigation. P13 mentioned that while \bma{} can indicate the presence of obstacles like stairs, it does not provide essential details such as the distance to these obstacles or their characteristics, which are typically discerned through O\&M tools like white canes or guide dogs.


\begin{quote}
    \textit{``[\bma] says, you know, `stairs in front,' and it's like, `Okay, that's great, but where are they? How far are they? Are they going up? Are they going down? Is there a railing?' which would be information that the dog or the cane could tell you. So, I would say use it as a tool along with, but definitely not by itself.''} (P13)
\end{quote}


In summary, \bma{} boosts spatial awareness and independence, although some participants question its practicality and safety during navigation. However, there is consensus that \bma{} can only complement, rather than replace participants' O\&M skills. 


%%%%%%%%%%%
%%%%%%%%%%%
\subsection{Engaging in Social Interactions}

In this section, we assess how \bma{} supports various social engagements, including digital and physical human interactions, as well as human-animal interactions. It highlights \bma's role in enhancing users' social experiences across different settings.



%%%%%%%%%
\subsubsection{Digital Human Social Interactions}
\label{digital}

Participants leveraged \bma{} to engage in social interactions with blind and sighted people on social media by using it to describe pictures that are posted on social media (P1-4, P7, P10, P11), check the quality of pictures that participants intend to post on social media (P2, P4, P9), and generate descriptions of their own pictures to post on social media (P2, P3, P7).



\paragraph{Artifact as Cognitive Support:}
Pictures posted on social media often lack alt text, which describes an image's content and is accessible through screen readers.
% 
Seven participants (P1-4, P7, P10, P11) value \bma's detailed interpretations of images posted on social media that are missing alt text, allowing them to fully comprehend the visual content. For example, P7 illustrated the effectiveness of \bma{} in contrast to Facebook's AI image description tool. 
% 
While Facebook AI might provide a vague description such as \textit{``picture of five people,''} \bma{} provides a vivid depiction, such as describing a scene with someone skiing on a mountain alongside a visible ski lift. 
% \textit{``exactly what [people] are doing in the picture,''} including elements of the background. 
This level of detail enhanced P7's immersive experience, 
as she put it, \textit{``[\bma] gives me a clearer picture of what's around, especially in pictures of, you know, the scene. I can visualize it as to the point where I'm almost there.''}




%%%%%%%%%%%%%%%%
% check and post pictures 

Furthermore, \bma{} not only assists participants as recipients but also empowers them to become active contributors, enhancing their engagement on social media platforms. First, \bma{} supports participants in ensuring the quality and appropriateness of images they intend to post on social media (P2, P4, P9). It helps them check content clarity and composition to select suitable images. 
% 
Second, \bma{} assists in creating accessible alt text (P2, P3, P7), facilitating easier access for other visually impaired users on social media. 
It allows participants to add personalized details such as familiar names or specific characteristics. 
% , enhancing the descriptions' relevance and accessibility.




\paragraph{Individual Adaptation and Cognitive Strategies:}
The adoption of \bma{} has altered the social media behavior of participants, enhancing their confidence and engagement. By understanding the visual content of images, participants like P10 are more confident in posting pictures, overcoming previous hesitations due to uncertainty about the visual aspects of their posts: \textit{``Before, I was very shy to post pictures because I didn't know the visual description of them.''} 
% 
This tool also enables them to engage more actively with social media content. For instance, they can now provide detailed comments on friends' photos (P7) and use the content as a basis for conversations (P1, P3), achieving a level of social interaction similar to that of sighted users. 

% Participants can elaborate more detail with \bma, thus gain similar engagement on social media as sighted people because of mitigating the barrier of not enough description for visual content. 
% Participants were able to give more reactions, like \textit{``comment on them''} (P7), to their friends' photos on social media. Also, the content of others' image posts is \textit{``a nice talking point''} (P3), where participants can \textit{``have something to talk to them about because you know what pictures they put up''}(P1)


%%%%%% others post images

Moreover, \bma's accurate image descriptions also affect the behaviors of sighted individuals who share images with participants. It alleviates the pressure on sighted people to provide perfect descriptions, thereby facilitating more frequent and meaningful interactions. As noted by P3, \textit{``Sighted people who now feel like they can send pictures without the pressure of having to describe it perfectly,''} indicating that \bma{} helps bridge the communication gap between visually impaired and sighted communities.


In summary, \bma{} provides detailed image descriptions for participants, enabling them to access visual content on social media platforms. This capability allowed visually impaired and sighted users to interact more confidently and effectively in digital human interactions, promoting enhanced social engagement.



%%%%%%%%%%%%%
\subsubsection{Physical Human Social Interactions}
\label{physical}

\bma{} has been utilized for parenting (P4, P8, P9), facilitating gift exchanges (P2, P9, P12), and helping identify puzzles to play with families (P14). 


\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{images/physical social.png}
\caption{Image descriptions of a family celebration, provided by P9.}
\end{figure}



\paragraph{Artifact as Cognitive Support:}
In their parenting roles, participants (P4, P8, P9) effectively engaged \bma{} to offload the cognitive tasks of visual perception. They utilized \bma{} to describe and verify the appearance of their children, focusing on attributes like hair texture, skin complexion, and the styles and colors of clothing. This enabled them to dress their children appropriately. 
% [discussion] demonstrating how \bma{} extends their sensory capabilities into the visual domain. 
Similarly, P9 employed \bma{} to read and label books in Braille, enhancing her ability to contextualize stories and interact more engagingly with her child. 



\bma{} also facilitates enhanced engagement within family settings by providing detailed descriptions. P14 utilized \bma{} to differentiate between various puzzles by describing the images on the boxes, such as \textit{``whether it was a puzzle, a scene of cats, or a scene of bears.''} This capability is particularly notable when compared to human assistants, as P14 pointed out that \bma{} offers access to visual details that sighted family members often take for granted. For example, \bma{} read the text from the box specifying which piece needed to be placed in the center, a detail not initially provided by human assistants. In this context, \bma{} offloads the cognitive load associated with visual distinction, enabling P14 to participate more fully in family activities.

% \begin{quote}
%     \textit{``When used correctly, \bma{} can kind of foster a sense of connection with humans. It doesn't replace them but as someone who is low-vision, it allows me to have maybe more pre-information about something before I talk about it with my family or friends.''} (P14)
% \end{quote}


Despite its advantages, \bma{} has certain limitations that can hinder its effectiveness in providing goal-oriented information. P14's experience with a puzzle box illustrates this issue. While \bma{} could identify general shapes, it sometimes lacked the specificity required for more nuanced tasks.
% 
% In this instance, \bma{} read the text from the back of the puzzle box, indicating which piece should be placed in the center of the puzzle. When P14 asked for additional details to locate the center piece, \bma{} replied that it was square. However, this answer was insufficient because there were many square pieces, making it challenging to determine the correct one from the given description. 



\begin{quote}
    \textit{``When \bma{} read me the text of the box on the back of the puzzle that said, you know, this particular piece should be in the center of the puzzle. As a follow-up question I asked, `Could I have more information about the piece in the center?' And it said, `This piece is a square piece,' but I mean, there were many different square pieces, so I could not tell from that.''} (P14)
\end{quote}
This example shows that although \bma{} can process visual information, it may not always provide the level of detail needed to accomplish participants' goals. 





\paragraph{Individual Adaptation and Cognitive Strategies:}

The detailed visual interpretation capability of \bma{} enables participants to engage in more meaningful social interactions.
This adaptation was particularly evident in their approach to gift exchanges, which became more personalized and thoughtful. For example, P2 ensured that the price tags were removed from Christmas gifts before wrapping them, and P9 used \bma{} to read party invitations and prepare gifts that matched the theme. 

% [discussion: This capability underscores how \bma{} offloads the cognitive load of reading and interpreting visual information, allowing participants to engage more fully in social rituals.]


P12 used \bma{} to describe Christmas gifts, explaining that reading cards with \bma{} \textit{``makes it a more meaningful experience with other people.''}
% 
P12's experience illustrates how \bma{} enhances individual perception and, consequently, genuine social engagement. Before using \bma, opening Christmas cards was a performative act—pretending happiness despite not being able to see or understand the card's content. 
With \bma, P12 could capture the card's visual and textual details, allowing for authentic reactions to the messages. 
% This change transforms his interactions from a superficial act to a more genuine, joyful connection with others.

% {\color{blue}
% \begin{quote}
% \textit{``It definitely improves the quality of interactions around other people. And I would say quality of life in a sense, because, you know, when I get a Christmas card now, it's not like a dreaded, you know, I have to open it and act like I'm happy that I got it. Because I can't see it. Now I can actually take a picture of it and understand what it is.''} (P12)  
% \end{quote}
% }

In addition to enhancing individual perception, \bma{} plays a role in decision-making within physical social engagement. P14 highlighted this when describing her use of \bma{} to select a puzzle:
\textit{``I wanted part of my decision of putting a puzzle together to be, `Let me decide from a description of what the puzzles are that somebody could see on the box.'''} 
% 
P14 stressed the importance of this autonomy, noting that her decision to engage in the puzzle activity was enriched by having access to the same visual information that sighted people see on the box.

% [discussion] This autonomy is an essential component of distributed cognition, where external tools allow individuals to take control of their actions and reasoning, enhancing their overall engagement in social settings.


% [discussion] These examples underscore how \bma{} serves as a cognitive tool that not only offloads the tasks of visual perception and memory but also enhances individual reasoning and decision-making within social contexts. By extending sensory capabilities, \bma{} allows participants to engage more fully and independently in their social environments, reshaping their interactions and cognitive strategies.


In summary, \bma{} provided detailed visual interpretations that enabled participants to perform tasks independently and interact more authentically in physical social interactions. For example, participants used \bma{} to enhance engagements in family activities through parenting and gift exchanging. They also used \bma{} to facilitate decision-making and autonomy in choosing puzzles. 



%%%%%%%%%%%%%
\subsubsection{Human-Animal Interactions}
\label{animal}

Nine participants (P2, P4, P5, P8-11, P13, P14) utilized \bma{} to take leisure pictures of animals, including cats, dogs, birds, and horses, to know their status. 


\begin{figure}[t!]
\centering
\includegraphics[width=0.4\textwidth]{images/human animal.png}
\caption{Image description of a dog, provided by P9.}
\end{figure}

\paragraph{Artifact as Cognitive Support:}
Participants employed \bma{} to enhance their perception of animals' states and behaviors, which are critical aspects of interacting safely and effectively with animals. \bma{} acted as an external cognitive aid that enabled participants to access visual information. 
% 
For example, participants (P5, P10, P11) used \bma{} to grasp nuances such as animals’ facial expressions, activities, and body language. P10, in particular, highlighted the utility of \bma{} during walking her dog, where she put it, \textit{``Sometimes it's hard for me to know if the dog is peeing or what the dog is doing.''}


Furthermore, P11's application of \bma{} in a farm setting exemplifies its role in enhancing awareness and safety for human-animal interactions. He uses the artifact to determine the locations and directions of mini horses in stalls for safety measure, like \textit{``Is the horse's head facing towards me or away from me? Is the horse turned towards the side? Based on where I am, where is its tail or hind, or its back end located?''}
% 
P11 shared an incident where he was between two horses and was accidentally kicked by a mini horse that reacted jealously to his attention towards another larger one. 
% 
This incident underscores the necessity of \bma{} in preempting dangerous situations, thus allowing P11 to take preventive measures. For example, using lead rope to \textit{``turn [the mini horse's] head the other way, and change her direction, get her focus back on me so she wouldn't have kicked me.''}

% [discussion:] how \bma{} supports strategic reasoning and safety in real-time interactions.




\paragraph{Individual Adaptation and Cognitive Strategies:}

While \bma{} provides valuable information in human-animal interactions, participants often adapted the tool's outputs to align with their own perceptions and combine them with other sensory information to ensure accuracy and safety.


P5, for example, emphasized personal judgment over the tool's subjective interpretations. She preferred the flexibility to override \bma's assumptions about her dogs' expressions. This strategy allowed P5 to balance AI-based interpretations with her subjective inputs, reinforcing her sense of control in understanding pet behaviors.
\begin{quote}
    \textit{``I like having more control over the description. So I like the ability to edit that. Some blind people think, `How does it know that the dogs are happy? Why does it assume?' Some people don't like that it's making assumptions about the picture. I like having access to that information, but I like to be able to change it if I want.''} (P5)
\end{quote}

% control, competence - can change the description

P11 integrated visual interpretations from \bma{} with auditory, tactile, and olfactory cues to bolster safety during interactions with horses. He supplemented this information by consulting AI tools like ChatGPT, which guided him on how to interact safely based on sensory cues. For instance, he asked for advice on how to handle horses safely without sight, such as maintaining close contact and physical awareness of the horse's movements. This approach demonstrates how P11 skillfully combined technological insights with his sensory perceptions to ensure safety and navigate his interactions with horses effectively.


In summary, participants delegated the visual perception of monitoring the animal status to \bma. They further adapted \bma's output by incorporating their own perceptions and other sensory information to ensure accuracy and safety.




% \begin{quote}
%     \textit{``And you also want to use \bma{} to see when you go up to a stall, because sometimes they move horses around so you want to know, `is the same horse in the stall? or is there a different one? And is the horse big? Is it small? is it medium sized? Where is it? is it in the front? Is it in the back of the stall? You know which direction is it facing? Is it safe for me to go in or not?''} (P11)
% \end{quote}


% [integration with chatgpt] ensure safety based on hearing touching smelling feedback
% No, because I've used other AI. I've used ChatGPT, which is what Be My AI runs off of. So I would go and spend time with horses. And then if I didn't understand what I was hearing or touching or smelling or something that they did, I would go when asked ChatGPT, I would say you know I'm totally blind, the horse behaved this way. How can I interact with a horse you know, safely without being kicked? 

% Oh, a whole lot. Especially, I mean if I wouldn't have had Be My AI and other AI related tools. It would have probably been a lot more difficult for me to spend time with and interact with horses because I couldn't have told the AI, “I'm totally blind, give me tips on how to be safe around horses. How can I avoid being ticked as a totally blind person?” And it would tell me all those things it would say, “Well, if you're totally blind, you want to stay as close to the horse as possible. Keep your hand on it, especially when you're walking around it.” Things like that.


% {\color{red}
% summary -- what characteristics is supporting cognition
% }

==> sections/outline.tex <==
\section{Findings}

\subsection{Context awareness}
\subsubsection{physical environment}
\paragraph{tbd, explanation}

\paragraph{example 1: spatial memory, mental model}


\paragraph{example 2: other sensory cues}


\paragraph{implication}



\subsubsection{social cues}

\paragraph{tbd}

\paragraph{example 1: Physical Human Social Interactions}

\paragraph{Example 2: human-animal interactions}

\paragraph{implication}





\subsubsection{Information Verification}

\paragraph{tbd, explanation}

\paragraph{example}


\paragraph{implication}



\subsection{Intent-oriented Capabilities}


\subsubsection{Subscription-based information retrieval}
\paragraph{tbd}


\paragraph{Example 1: eggshells}



\paragraph{Example 2: safety assessment when interacting with horses}



\paragraph{Example 3: customizable descriptions, vary on sight conditions}

\paragraph{implication}



\subsubsection{Agentic Interaction}

\paragraph{tbd}


\paragraph{example 1: user prompt}

\paragraph{implication}


\subsubsection{Real-time assistance}



\paragraph{tbd}

\paragraph{example 1: limited camera view}

\paragraph{Example 2: safety issues for mobility}


\paragraph{implication}



